Solving Neural Min-Max Games: The Role of Architecture, Initialization & Dynamics

Many emerging applications - such as adversarial training, AI alignment, and robust optimization - can be framed as zero-sum games between neural nets, with von Neumann-Nash equilibria (NE) capturing the desirable system behavior. While such games often involve non-convex non-concave objectives, empirical evidence shows that simple gradient methods frequently converge, suggesting a hidden geometric structure. In this paper, we provide a theoretical framework that explains this phenomenon through the lens of hidden convexity and overparameterization. We identify sufficient conditions - spanning initialization, training dynamics, and network width - that guarantee global convergence to a NE in a broad class of non-convex min-max games. To our knowledge, this is the first such result for games that involve two-layer neural networks. Technically, our approach is twofold: (a) we derive a novel path-length bound for the alternating gradient descent-ascent scheme in min-max games; and (b) we show that the reduction from a hidden convex-concave geometry to two-sided Polyak-{\L}ojasiewicz (P{\L}) min-max condition hold with high probability under overparameterization, using tools from random matrix theory.

==> main_results.tex <==
\section{Our Results}


Our main result concerning the order analysis for general, regularized hidden min-max games with strongly-convex-strongly-concave losses proceeds as follows: First, we bound the AltGDA path length by defining an appropriate Lyapunov potential function followed by upper bounding this potential function itself in terms of gradients of the min-max objective function. Afterwards, we ensure AltGDA trajectory stays close to the random initializations. Finally we find appropriate random initializations that ensure this. More importantly, finding this random initialization also provides us the amount of overparameterization needed.

\subsection{Bounding the AltGDA path length}
We will obtain a bound on the distance between $t$-th iterates and the saddle point $(\theta^*,\phi^*)$. % Before that, we will first make a note of a helper results.

% \subsubsection{Helper Results}
% \begin{theorem}[Lipschitzness of maximizers]
% Let function $f: X \times Y \rightarrow \mathbb{R}$ be an $\ell$-smooth function with $f(\theta, \cdot)$ satisfying the PŁ-condition with parameter $\mu_2$ for all $x \in \mathbb{R}^m$. Then, for any $\theta_1, \theta_2 \in \mathbb{R}^n$ and the corresponding points $\phi^*(\theta_1), \phi^*(\theta_2) \in \mathbb{R}^n $ defined as
% \begin{eqnarray*}
% \phi^*(\theta_1) \coloneqq \arg\max_{\phi \in \mathbb{R}^n} f(\theta_1, \phi) \\
% \phi^*(\theta_2) \coloneqq \arg\max_{\phi \in \mathbb{R}^n} f(\theta_2, \phi)
% \end{eqnarray*}
% we have that
% \[
% \| \phi^*(\theta_1) - \phi^*(\theta_2) \| \leq L_* \| \theta_1 - \theta_2 \|,
% \]
% where $L_* \coloneqq \frac{\ell}{\mu_2}$.
% \end{theorem}

\subsubsection{Defining Lyapunov Potential Function and Bounding It}
Since our focus is on min-max problems, we define the classical min-max optimality gap as the Lyapunov potential function: $P_t \triangleq U_t + \lambda W_t,\;\forall t\geq 0$  where 
\begin{align}
    U_t & \triangleq \Phi(\theta_t) - \Phi^* \\
    W_t & \triangleq  \Phi(\theta_t) - f(\theta_t, \phi_t)
\end{align}
Here, $\Phi(\theta) \triangleq \max_{\phi} f(\theta,\phi)$.

The following result by \citeauthor{yang2020global} \cite{yang2020global} (Theorem 3.2) tells us the distance of AltGDA iterates $(\theta_t,\phi_t)$ at any instant $t$ can be upper-bounded in terms of the potential $P_t$ at $t=0$:
\begin{lemma}[Theorem 3.2 in \cite{yang2020global}]
    \label{lem:agda-dist-to-saddle}
    Suppose the min-max objective function $f(\theta,\phi)$ satisfies Assumptions \ref{ass:min-max-obj-assumptions} and the two-sided PŁ-condition with $(\mu_1,\mu_2)$. Define the Lyapunov potential $P_t = U_t + \frac{1}{10} W_t$. If we run AltGDA with $\eta_1 = \frac{\mu_2^2}{18L_{f,grad}^{3}}$ and $\eta_2 = \frac{1}{L_{f,grad}}$, then 
    \begin{equation}
        \lVert \theta_{t+1} - \theta_t \rVert + \lVert \phi_{t+1} - \phi_t \rVert \leq \sqrt{\alpha} c^{t/2} \sqrt{P_0}
    \end{equation}
    where $\alpha = \frac{2(1+\eta_2^2 L_f^2) \eta_1^2 L^2}{\mu_1} + \frac{20(1+\eta_2^2 L_f^2) \eta_1^2 L_f^2 + 20 L_f^2 \eta_2^2}{\mu_2}$, $L = L_f + \frac{L_f^2}{\mu_2} $, and $c = 1 - \frac{\mu_1 \mu_2^2}{36 (L_{f,grad})^3}$.
\end{lemma}

Moreover, in order to obtain an upper bound on the AltGDA path length that takes into account the properties of our neural network at random initializations and throughout the network training, we will bound the AltGDA path length by upper-bounding the Lyapunov potential at time $t=0$ in terms of the gradients and values of the objective function at the initialization points $(\theta_0, \phi_0)$.

\begin{lemma}[Upper bounding potential $P_t$]
\label{lem:potential-upper}
    Suppose the min-max objective function satisfies Assumption \ref{ass:min-max-obj-assumptions} and the two-sided PŁ-condition with $(\mu_1,\mu_2)$. Then, we get the following upper bound for the Lyapunov potential $P_t$:
    \begin{equation}
        \label{eq:P_t-upper-bound}
        P_t = U_t + \lambda W_t \leq  L_f \left(C_1 \cdot \lVert \nabla_{\theta} f(\theta_t, \phi_t) \rVert + C_2 \cdot \lVert \nabla_{\phi} f(\theta_t, \phi_t) \rVert \right)
    \end{equation}
    where $C_1 = \sqrt{\frac{2}{\mu_1^3}}$ and $C_2 = \sqrt{\frac{2}{\mu_2^3}}(1+\lambda)L_f $.
\end{lemma}
\begin{proof}
Since $f$ is $L_f$-Lipschitz and satisfies 2-sided PŁ-condition, we can obtain the following bound for $W_t$:
\begin{align}
        W_t & = \max_\phi f(\theta_t, \phi) - f(\theta_t, \phi_t) \nonumber \\
        & = f(\theta_t, \phi^*(\theta_t)) - f(\theta_t, \phi_t) \nonumber \\ 
        & \leq L_f \lVert \phi^*(\theta_t) - \phi_t \rVert \nonumber \\
        & \overset{(QG)}{\leq} \frac{2 L_f}{\mu_{2}} \cdot \sqrt{f(\theta_t, \phi^*(\theta_t)) - f(\theta_t, \phi_t)} \nonumber \\
        \implies W_t & \overset{(PL)}{\leq} L_f \cdot C'_2 \cdot \lVert \nabla_{\phi} f(\theta_t, \phi_t) \rVert \nonumber \\
        \label{eq:W0}
    \end{align}
where $C'_2 = \sqrt{\frac{2}{\mu_2^3}}$. For $U_0$, we can say that:
    \begin{align}
        U_0 & = f(\theta_t, \phi^*(\theta_t)) - f(\theta^*, \phi^*) \\
        & \leq f(\theta_t, \phi^*(\theta_t)) - f(\theta^*, \phi_t) \;\;\;\;(f(\theta^*, \phi) \leq f(\theta^*, \phi^*) \;\forall \phi)\\
        & \leq f(\theta_t, \phi^*(\theta_t)) - f(\theta^*(\phi_t), \phi_t) \;\;\;\;(\because f(\theta^*, \phi_t) \geq f(\theta^*(\phi_t), \phi_t)) \\
        & \leq L_f \lVert \theta_t - \theta^*(\phi_t) \rVert + L_f \lVert \phi^*(\theta_t) - \phi_t \rVert \\
        & \overset{(QG)}{\leq} \frac{2 L_f}{\mu_{1}} \cdot \sqrt{f(\theta_t, \phi_t) - f(\theta^*(\phi_t), \phi_t)} +  \frac{2 L_f}{\mu_{2}} \cdot \sqrt{f(\theta_t, \phi^*(\theta_t)) - f(\theta_t, \phi_t)} \\
        & \overset{(PL)}{\leq} L_f \left(C_1 \cdot \lVert \nabla_{\theta} f(\theta_t, \phi_t) \rVert + C'_2 \cdot \lVert \nabla_{\phi} f(\theta_t, \phi_t) \rVert \right) \label{eq:U0_bound}
    \end{align}
where $C_1 = \sqrt{\frac{2}{\mu_1^3}}$. By Equations \eqref{eq:W0}, and \eqref{eq:U0_bound} above, we have that 
    \begin{align}
    \label{eq:P_0-upper-gradients}
        P_t & \leq \Bigg( L_f (C_1 \cdot \lVert \nabla_{\theta} f(\theta_t, \phi_t) \rVert + C'_2 \cdot \lVert \nabla_{\phi} f(\theta_t, \phi_t) \rVert ) + \lambda \cdot L_f \cdot C'_2 \cdot \lVert \nabla_{\phi} f(\theta_t, \phi_t) \rVert \Bigg)
    \end{align}
\end{proof}

\subsubsection{Ensuring the AltGDA trajectory stays close to the random initializations ($\mathbf{\theta_0}, \mathbf{\phi_0}$)}

Based on Lemma \ref{lem:agda-dist-to-saddle} above, we can do the following simple calculation about the length of the AltGDA trajectory: let $T$ denote the first iteration such that $(\theta_t, \phi_t) \not\in \mathcal{B}((\theta_0,\phi_0), R)$. Then, the length of the GDA trajectory is upper bounded by
        \begin{align}
            \ell(T) & \triangleq \sum_{t=0}^{T-1} \lVert (\theta_{t+1}, \phi_{t+1}) - (\theta_t, \phi_t) \rVert \\
            & \leq  \sum_{t=0}^{T-1} \lVert \theta_{t+1} - \theta_t \rVert + \lVert \phi_{t+1} - \phi_t \rVert \\
            & \leq \sqrt{2\alpha_1} \sum_{t=0}^{\infty} c^{t/2} P_{0}^{1/2} \;\; (\text{By Lemma }\ref{lem:agda-dist-to-saddle}) \\
            & = \frac{\sqrt{2\alpha'_1}}{1 - \sqrt{c}} \cdot \sqrt{P_0}\\
            & \overset{\text{want}}{<} R \;( = R/2 \text{, say})\\
            \implies P_0 & = \kappa R^2 \label{eq:P0-radius-bound}
        \end{align}
where $\alpha' = 2\alpha'_1 = 2 \cdot \left[ \frac{2(1+\eta_2^2 L_{f,grad}^2) \eta_1^2 L^2}{\mu_1} + \frac{20(1+\eta_2^2 L_{f,grad}^2) \eta_1^2 L_{f,grad}^2 + 20L_{f,grad}^2 \eta_2^2}{\mu_2}\right]$, $c = 1 - \frac{\mu_1 \mu_2^2}{36 L_{f,grad}^3}$ and $\kappa = \frac{(1-\sqrt{c})^2}{8\alpha'_1}$.

\subsection{Warmup: Safe Initialization}
\label{subsec:warmup-safe-init}

As a starting point, let's focus on the following simplest setting: using latent strategies for solving hidden bilinear min-max games where the players play their strategies by transforming them through neural network whose weight matrices are randomly initialized and fixed. This is exactly the framework analysed by Sakos et al. \cite{sakos2023exploiting}. However, the authors there assume that the network initializations are such that the network's Jacobian is non-singular and continues to remain so for the entire trajectory of the parameter iterates. Here, we will prove that this assumptions holds true with high probability when using a 1-hidden-layer neural network. Before we proceed, for this warmup case, our objective function, $f(\theta,\phi)$, has been defined as follows ($ \varepsilon > 0 $) for a given payoff matrix, $A$:
    \begin{equation}
    \label{eq:warmup-min-max-objective}
        f(\theta,\phi) = h(\theta)^\top A g(\phi) + \frac{\varepsilon}{2} \lVert h(\theta) \rVert^2 - \frac{\varepsilon}{2} \lVert g(\phi) \rVert^2
    \end{equation}
Here, the neural networks $h,g$ are defined as $h(\theta) = W_2^{(h)} \psi(W_1^{(h)} \theta)$ and $g(\phi) = W_{2}^{(g)} \psi(W_1^{(g)} \phi)$ where $W_k^{(h)} \sim \mathcal{N}(0,(\sigma_k^{(h)})^2 I_{d_{k}^{(h)} \times d_{k-1}^{(h)}})$ and $W_k^{(g)} \sim \mathcal{N}(0,(\sigma_k^{(g)})^2 I_{d_{k}^{(g)} \times d_{k-1}^{(g)}})$, $k\in\{1,2\}$, and $\psi$ is a differentiable activation function (e.g. GeLU, sigmoid, tanh). Therefore, the partial derivatives w.r.t. $\theta$ and $\phi$ will be as follows:
    \begin{align}
        \nabla_{\theta} f(\theta, \phi) & = J_{h(\theta)}^\top A g(\phi) + \varepsilon J_{h(\theta)}^\top h(\theta) \\
        \nabla_{\phi} f(\theta, \phi) & = J_{g(\phi)}^\top A^\top h(\theta) - \varepsilon J_{g(\phi)}^\top g(\phi)
    \end{align}
\begin{remark}(Why $\ell_2$-regularization?)
    For the case of bilinear games, we know from the work of \citeauthor{bailey2020finite} \cite{bailey2020finite} that if we are using fixed step-sizes for AltGDA, then the strategies for the two players exhibit Poincar\'e recurrence — they return arbitrarily close to their initial positions infinitely often. For the time being, even though we are considering hidden bilinear games for our work here, let's assume the neural network mappings are identity mappings. That is, $h(\theta) = \theta $ and $g(\phi) = \phi$ $\forall \theta,\phi$. Then, by adding strongly-convex-strongly-concave regularization, our min-max objective now satisfies the 2-sided PŁ-condition \cite{yang2020global}:
    \[
        \min_{\theta} \max_{\phi} \left\{ \theta^\top A \phi + \frac{\varepsilon}{2} \lVert \theta \rVert^2 - \frac{\varepsilon}{2} \lVert \phi \rVert^2 \right \}
    \]
    Thus, because this function satisfies 2-sided-PŁ condition, by convergence results of \citeauthor{yang2020global} \cite{yang2020global}, we see that AltGDA iterates with fixed step-sizes convergence and doesn't exhibit any cycles for our min-max objective.
\end{remark}
    
Therefore, we can now bound $P_0$ as follows:
    \begin{align}
    P_0 & \leq \Bigg( L_f (C_1 \cdot \lVert J_{h(\theta_0)}^\top \rVert \cdot (A g(\phi_0) \rVert + \varepsilon\lVert h(\theta_0) \rVert) + C'_2 \cdot (1 + \lambda) \cdot \lVert J_{g(\phi_0)}^\top \rVert \cdot (\lVert A^\top h(\theta_0) \rVert + \varepsilon\lVert g(\phi_0) \rVert)) \Bigg) \nonumber \\
        & \leq \Bigg( L_f (C_1 \cdot \lVert J_{h(\theta_0)}^\top \rVert \cdot (\lVert A\rVert \lvert g(\phi_0) \rVert + \varepsilon\lVert h(\theta_0) \rVert) + C'_2 \cdot (1 + \lambda) \cdot \lVert J_{g(\phi_0)}^\top \rVert \cdot (\lVert A^\top \rVert \lVert h(\theta_0) \rVert + \varepsilon\lVert g(\phi_0) \rVert)) \Bigg) \nonumber \\
    \implies P_0 & \leq \lVert h(\theta_0) \rVert \cdot (\varepsilon L_f C_1 \lVert J_{h(\theta_0)}^\top \rVert + L_f C'_2 (1+\lambda) \lVert J_{g(\phi_0)}^\top \rVert \lVert A^\top \rVert) \nonumber \\ 
    & + \lVert g(\phi_0) \rVert \cdot (L_f C_1 \lVert J_{h(\theta_0)}^\top \rVert \lVert A \rVert +\varepsilon C'_2 (1+\lambda) \lVert J_{g(\phi_0)}^\top \rVert) \nonumber\\
    \implies P_0 & \leq  \lVert h(\theta_0) \rVert \cdot (\varepsilon L_f C_1 \sigma_{\max}(J_{h(\theta_0)}) + L_f C'_2 (1+\lambda)\sigma_{\max}(A) \sigma_{\max}(J_{g(\phi_0)})) \nonumber \\
        & + \lVert g(\phi_0) \rVert \cdot (L_f C_1 \sigma_{\max}(A)\sigma_{\max}(J_{h(\theta_0)}) +\varepsilon C'_2(1+\lambda)\sigma_{\max}(J_{g(\phi_0)})) \label{eq:P_0-bound-1}
    \end{align}
where $\theta_0, \phi_0$ are random parameter initializations for the neural networks $h$ and $g$ respectively.

Thus, to ensure that AltGDA trajectory doesn't steer too far away from the random initializations $(\theta_0,\phi_0)$, we need to control the two terms in the upper bound of the potential $P_0$ (Equation \ref{eq:P_0-bound-1}). In other words, we want to find initializations $(\theta_0,\phi_0)$ such that the neural network outputs $h(\theta_0)$ and $g(\phi_0)$ are small enough to ensure the potential at $t=0$ is small thereby ultimately keeping the AltGDA trajectories contained within the ball $\mathcal{B}((\theta_0,\phi_0), R)$. Here, we will define the ball radius $R$ as $R = \frac{\mu_{\text{Jac}}}{2\beta}$ with $\mu_{\text{Jac}} = \min\{\mu_{\text{Jac}}^{(h)}, \mu_{\text{Jac}}^{(g)}\}$ and $\beta = \max\{\beta_h,\beta_g\}$ where $\mu_{\text{Jac}}^{(h)}, \mu_{\text{Jac}}^{(g)}$ are lower bounds for the smallest singular value and $\beta_h$, $\beta_g$ are Lipschitz constant of the neural network Jacobian for networks $h$ and $g$, respectively. This radius $R$ is chosen so that if we can ensure that the Jacobian singular values are bounded away from zero and also bounded from above, then they continue to remain so within $\mathcal{B}((\theta_0,\phi_0), R)$ (Lemma 1 of \citeauthor{song2021subquadratic} \cite{song2021subquadratic}).



Using well-known results from random matrix theory about minimum and maximum singular values of random Gaussian matrices, we can provide high probability bounds for the minimum and maximum singular values of the neural network Jacobian for the networks $h$ and $g$ as shown below in Lemma \ref{lem:warmup-jacobian-singular-whp}.

\begin{lemma}
    \label{lem:warmup-jacobian-singular-whp}
    Consider a neural network $h$ with parameters $\theta\in\mathbb{R}^{d_0^{(h)}}$ defined as $h(\theta) = W_{2}^{(h)} \psi(W_{1}^{(h)}\theta)$ where $W_{k}^{(h)} \in \mathbb{R}^{d_{k}^{(h)} \times d_{k-1}^{(h)}}$ ($k\in \{1,2\}$), $(W_{1}^{(h)})_{i,j} \sim \mathcal{N}(0,(\sigma_{1}^{(h)})^2)\;\forall i,j$ , $(W_{2}^{(h)})_{k,l} \sim \mathcal{N}(0,(\sigma_{2}^{(h)})^2 )\;\forall k,l$ and $\psi$ is the GeLU activation function with $d_{1}^{(h)} \geq 256 d_{0}^{(h)}$, $d_{1}^{(h)} \geq 256 d_{2}^{(h)}$ and $(\sigma_{1}^{(h)})^2 < \frac{\pi}{4Cd_{1}^{(h)} \lVert \theta \rVert^2}$. Then the minimum singular value of the Jacobian $J_{h(\theta)} = \frac{\partial h(\theta)}{\partial \theta}$ is lower bounded as
    \begin{equation}
        \label{eq:warmup-jac-min-sing}
        \sigma_{\min}(J_{h(\theta)}) > \frac{\sigma_{1}^{(h)} \sigma_{2}^{(h)} d_{1}^{(h)}}{16} \cdot \left( \frac{1}{2} - \sigma_{1}^{(h)}\lVert \theta\rVert \sqrt{\frac{Cd_{1}^{(h)}}{\pi}} \right)
    \end{equation}
    w.p $\geq 1 - 2e^{-\frac{d_{1}^{(h)}}{64}} - e^{-Cd_{1}^{(h)}}$. The maximum singular value of $J_{h(\theta)}$ is upper bounded as
    \begin{equation}
        \label{eq:warmup-jac-max-sing}
        \sigma_{\max}(J_{h(\theta)}) < 3.47\sigma_{1}^{(h)} \sigma_{2}^{(h)} d_{1}^{(h)}
    \end{equation}
    w.p. $\geq 1 - 2e^{-\frac{d_{1}^{(h)}}{64}}$.
\end{lemma}
\begin{proof}
    By Theorem 4.6.1 in \cite{vershynin2018high}, we get $\sigma_1 (\sqrt{d_{1}^{(h)}} - 4(\sqrt{d_{0}^{(h)}} + t)) \leq \sigma_{\min}(W_{1}^{(h)}) \leq \sigma_{\max}(W_{1}^{(h)}) \leq \sigma_{1}^{(h)} (\sqrt{d_{1}^{(h)}} + 4(\sqrt{d_{0}^{(h)}} + t)) $ w.p. $\geq 1 - 2e^{-t^2}$. By choosing $t = \frac{1}{8}\sqrt{d_{1}^{(h)}}$, we get $\sigma_{1}^{(h)} (\frac{1}{2} \sqrt{d_{1}^{(h)}} - 4\sqrt{d_{0}^{(h)}}) \leq \sigma_{\min}(W_{1}^{(h)}) \leq \sigma_{\max}(W_{1}^{(h)}) \leq \sigma_{1}^{(h)} (\frac{3}{2}\sqrt{d_{1}^{(h)}} + 4\sqrt{d_{0}^{(h)}})$ w.p. $\geq 1 - 2e^{-d_{1}^{(h)}/64}$. If we set $d_{1}^{(h)} \geq 256 d_{0}^{(h)}$, we get $(\frac{1}{2} \sqrt{d_{1}^{(h)}} - 4\sqrt{d_{0}^{(h)}}) \geq \frac{1}{4} \sqrt{d_{1}^{(h)}}$ and $\frac{3}{2}\sqrt{d_{1}^{(h)}} + 4\sqrt{d_{0}^{(h)}} \leq \frac{7}{4}\sqrt{d_{1}^{(h)}}$. Therefore, we get that w.p. $\geq 1 - 2e^{-\frac{d_{1}^{(h)}}{64}}$,
    \[
    \frac{1}{4}\sigma_{1}^{(h)} \sqrt{d_{1}^{(h)}} \leq \sigma_{\min}(W_{1}^{(h)}) \leq \sigma_{\max}(W_{1}^{(h)}) \leq \frac{7}{4}\sigma_{1}^{(h)}\sqrt{d_{1}^{(h)}}.\]
    For the case of $W_2^{(h)}$, because we have $d_{2}^{(h)} < d_{1}^{(h)}$, for the bounds to be non-vacuous, we will use analogous reasoning as that for $W_{1}^{(h)}$ above for $(W_{2}^{(h)})^\top$ with $t = \frac{1}{8}\sqrt{d_{1}^{(h)}}$ which yields w.p. $\geq 1 - 2e^{-\frac{d_{1}^{(h)}}{64}}$, $ \sigma_{2}^{(h)} (\frac{1}{2} \sqrt{d_{1}^{(h)}} - 4\sqrt{d_{2}^{(h)}}) \leq \sigma_{\min}((W_{2}^{(h)})^\top) = \sigma_{\min}(W_{2}^{(h)}) \leq \sigma_{\max}((W_{2}^{(h)})^\top) = \sigma_{\max}(W_{2}^{(h)}) \leq \sigma_2^{(h)} (\frac{3}{2}\sqrt{d_{1}^{(h)}} + 4\sqrt{d_{2}^{(h)}})$. Then, by setting $d_{1}^{(h)} \geq 256 d_{2}^{(h)}$, we get
    \[
        \frac{1}{4}\sigma_{2}^{(h)} \sqrt{d_{1}^{(h)}} \leq \sigma_{\min}(W_{2}^{(h)}) \leq \sigma_{\max}(W_{2}^{(h)}) \leq \frac{7}{4}\sigma_{2}^{(h)}\sqrt{d_{1}^{(h)}}
    \]
    Note that the Jacobian for the neural network $h(\theta)$ can be computed as
    \begin{equation}
        J_{h(\theta)} = \frac{\partial h(\theta)}{\partial \theta} = W_{2}^{(h)} \frac{\partial}{\partial z}\psi(z) W_{1}^{(h)} = W_{2}^{(h)} \Psi(W_{1}^{(h)} \theta) W_{1}^{(h)}
    \end{equation}
    where $z\coloneq W_{1}^{(h)} \theta$ and $\Psi(W_{1}^{(h)}\theta) = $ diag$(\psi'((W_{1}^{(h)}\theta)_1),\ldots, \psi'((W_{1}^{(h)}\theta)_{d_{1}^{(h)}}))$. Therefore, we can compute the minimum and maximum singular values for this Jacobian $J_{h(\theta)}$ by looking at its operator norm: $\lVert J_{h(\theta)} \rVert = \lVert W_{2}^{(h)} \Psi(W_{1}^{(h)}\theta) W_{1}^{(h)} \rVert$. Then, by properties of the operator norm, we see that $\lVert J_{h(\theta)} \rVert \geq  \sigma_{\min}(W_{2}^{(h)}) \lVert \Psi(W_{1}^{(h)}\theta) \rVert \sigma_{\min}(W_{1}^{(h)})$ and $\lVert J_{h(\theta)} \rVert \leq  \sigma_{\max}(W_{2}^{(h)}) \lVert \Psi(W_1^{(h)}\theta) \rVert \sigma_{\max}(W_1^{(h)})$. This further tells us that $\sigma_{\min}(J_{h(\theta)}) \geq \sigma_{\min}(W_2^{(h)}) \sigma_{\min}(\Psi(W_1^{(h)}\theta)) \sigma_{\min}(W_1^{(h)})$ and $\sigma_{\max}(J_{h(\theta)}) \leq  \sigma_{\max}(W_2^{(h)}) \sigma_{\max}(\Psi(W_1^{(h)}\theta)) \sigma_{\max}(W_1^{(h)})$. We can further simplify these lower and upper bounds for the Jacobian singular values by noting that since $\Psi(W_1^{(h)}\theta)$ is a diagonal matrix, $\sigma_{\min}(\Psi(W_1^{(h)}\theta)) = \underset{1\leq i \leq d_1^{(h)}}{\min}\;\psi'(z_i)$ and $\sigma_{\max}(\Psi(W_1^{(h)}\theta)) = \underset{1\leq i \leq d_1^{(h)}}{\max}\;\psi'(z_i)$ where $z_i = (W_1^{(h)}\theta)_i\;\forall i \in [d_1^{(h)}]$.
    
    Now, notice that $z = W_1^{(h)} \theta \sim \mathcal{N}(0, (\sigma_1^{(h)})^2 \lVert \theta \rVert_2^2 I_{d_1^{(h)}\times d_1^{(h)}})$. % Thus, for any $\epsilon > 0$, we have
    % \begin{align}
    %     P[A_1\theta > \epsilon] & = P[\forall i: (A_1\theta)_i > \epsilon] \\
    %     & = (P[(A_1\theta)_1 > \epsilon])^{d_1} \;\; (\because z_i = (A_1\theta)_i \overset{iid}{\sim} \mathcal{N}(0,\sigma_1^2 \lVert \theta\rVert_2^2)) \\
    %     & = (1 - P[(A_1\theta)_1 \leq \epsilon])^{d_1} \\
    %     & = (1 - \Phi(x))^{d_1} \;\;\left(x \coloneq \frac{\epsilon}{\sigma_1 \lVert \theta \rVert}, \Phi(x)=P[U \leq x] \text{ for } U\sim \mathcal{N}(0,1)\right)\\
    %     & \leq e^{-\frac{1}{2}d_1 x^2} \;\;(\text{Chernoff bound for Gaussian distribution}) \\
    %     & = e^{-\frac{\epsilon^2}{2\sigma_1^2\lVert \theta\rVert^2}d_1} \\
    %     & < e^{-cd_1} \;\;(\text{if } \epsilon > \sigma_1 \lVert \theta\rVert \sqrt{2c})
    %     % & = e^{d_1 \ln(1 - \Phi(x))} \;\;\left(\Phi(x)=P[U \leq x] \text{ for } U\sim \mathcal{N}(0,1) \right) \\
    %     % & \leq e^{-d_1 \Phi(x)} \;\;(\;\because \ln(1-y) \leq -y \;\;\forall y < 1) \\
    %     % & \leq e^{-\frac{d_1 x}{x^2 + 1} \frac{1}{\sqrt{2\pi}} e^{-x^2/2}}\\
    %     % & \left(\because \text{Mill's ratio for Gaussian distribution: } \Phi(x) \geq \frac{x}{x^2 + 1} \frac{1}{\sqrt{2\pi}} e^{-x^2/2}\right)  \\
    %     % & = 
    % \end{align}
Using the fact that GeLU's derivative, $\psi'$, is $L_{\psi'}$-Lipschitz with $L_{\psi'} = \sup_{x\in\mathbb{R}} |\psi''(x)| = \varphi(0) = \frac{1}{\sqrt{2\pi}}$ ($\varphi$ is standard normal PDF), we can appeal to concentration inequality for Lipschitz functions of Gaussian random variables and infer for $0 < \epsilon < 1/2$:
    \begin{align}
    P[\sigma_{\min}(\Psi(W_{1}^{(h)}\theta)) > \epsilon] & = P[\forall i : \psi'((W_1^{(h)}\theta)_i) > \epsilon] = (P[\psi'((W_1^{(h)}\theta)_1) > \epsilon])^{d_1^{(h)}} \\
    & = (P[\psi'((W_1^{(h)}\theta)_1) - 1/2 > \epsilon - 1/2])^{d_1^{(h)}} \\
    & = (P[\psi'((W_1^{(h)}\theta)_1) - E[\psi'((W_1^{(h)}\theta)_1)] > \epsilon - 1/2])^{d_1^{(h)}} \\
    (\because E[\psi'((W_1^{(h)}\theta)_1)] &= E[(W_1^{(h)}\theta)_1 \varphi((W_1^{(h)}\theta)_1)] + E[\Phi((W_1^{(h)}\theta)_1)] = 0 + 1/2) \\
    & (\varphi, \Phi \text{ are standard normal PDF \& CDF, resp.}) \\
    & \geq 1 - e^{-\frac{(1/2 -\epsilon)^2}{2 L_{\psi'}^2(\sigma_1^{(h)})^2\lVert\theta\rVert^2}} \\
    & (\because P[\psi'(z) \leq 1/2 - t] \leq e^{-\frac{\pi t^2}{(\sigma_1^{(h)})^2\lVert \theta\rVert^2}}; \text{ choose } t = 1/2 - \epsilon) \\
    & = 1 - e^{-Cd_1^{(h)}} \;(\text{if we set }\epsilon = 1/2 - (\sigma_1^{(h)} \lVert \theta\rVert\sqrt{Cd_1^{(h)}/\pi}))
    % P[\forall i: \psi'((A_1\theta)_i) > \epsilon] = (P[\psi'((A_1\theta)_1) > \epsilon])^{d_1} \;\; (\because z_i = (A_1\theta)_i \overset{iid}{\sim} \mathcal{N}(0,\sigma_1^2 \lVert \theta\rVert_2^2))
    \end{align}
    Therefore, as long as we have $(\sigma_1^{(h)})^2 < \frac{\pi}{4Cd_1^{(h)} \lVert \theta \rVert^2}$, we have w.p. $\geq 1 - e^{-Cd_1^{(h)}}$ that
    \begin{equation}
        \sigma_{\min}(\Psi(W_1^{(h)}\theta)) > \frac{1}{2} - \sigma_1^{(h)}\lVert \theta\rVert \sqrt{\frac{Cd_1^{(h)}}{\pi}}
    \end{equation}

    Combining all of this, we can say w.p. $\geq 1 - 2e^{-\frac{d_1^{(h)}}{64}} - e^{-Cd_1^{(h)}}$, we have:
    \begin{equation}
        \sigma_{\min}(J_{h(\theta)}) > \frac{\sigma_1^{(h)} \sigma_2^{(h)} d_1^{(h)}}{16} \cdot \left( \frac{1}{2} - \sigma_1^{(h)}\lVert \theta\rVert \sqrt{\frac{Cd_1^{(h)}}{\pi}} \right).
    \end{equation}
    And w.p. $\geq 1 - 2e^{-\frac{d_1^{(h)}}{64}}$, we have:
    \begin{equation}
        \sigma_{\max}(J_{h(\theta)}) < \left(\frac{7 \sqrt{d_1^{(h)}}}{4}\right)^2 \cdot 1.13\sigma_1^{(h)}\sigma_2^{(h)} < 3.47 \sigma_1^{(h)} \sigma_2^{(h)} d_1^{(h)}
    \end{equation}
    where we used the fact that $\max_{x\in\mathbb{R}} \psi'(x) = \psi'(\sqrt{2}) \approx 1.1289$.
    % By results from Rudelson et al. \cite{rudelson2009smallest}, since $A_1$ and $A_2$ are random rectangular matrices with independent Gaussian entries, we have that $\sigma_{\min}(A_k) \gtrsim \frac{1}{2}\sigma_k (\sqrt{d_{k}} - \sqrt{d_{k-1}})$ w.p. $\geq 1 - e^{-\frac{1}{8}(\sqrt{d_k} - \sqrt{d_{k-1}})^2}$ where $k\in\{1,2\}$. And by Theorem 4.4.5 in \cite{vershynin2018high}, we have that $\sigma_{\max}(A_k) \lesssim \sigma_k (2\sqrt{d_k} + \sqrt{d_{k-1}})$ w.p. $\geq 1 - e^{-\Theta(d_k)}$ where $k\in\{1,2\}$.
\end{proof}
\begin{lemma}
    \label{lem:warmup-jacobian-smoothness}
    Consider a neural network $h$ with parameters $\theta \in \mathbb{R}^{d_0^{(h)}}$ as defined in Lemma \ref{lem:warmup-jacobian-singular-whp} above. Then, w.p. $\geq 1 - 2e^{-\frac{d_1^{(h)}}{64}}$ the neural network $h$ is $\beta_h$-smooth where $\beta_h = \frac{1}{\sqrt{2\pi}}\cdot \frac{343(\sigma_1^{(h)})^2 \sigma_2^{(h)} (d_{1}^{(h)})^{3/2}}{64}$.
\end{lemma}
\begin{proof}
    In order to proof that $h$ is $\beta_h$-smooth, we need to show that Definition \ref{def:smooth-neural-net} holds true. For $\theta,\theta'\in \mathbb{R}^{d_0^{(h)}}$, we write
    \begin{align}
        \lVert J_{h(\theta)} - J_{h(\theta')} \rVert & \leq \lVert W_2^{(h)} \rVert \lVert \Psi(W_1^{(h)}\theta) - \Psi(W_1^{(h)}\theta') \rVert \lVert W_1^{(h)} \rVert \\
        & \leq \lVert W_2^{(h)} \rVert L_{\psi'} \lVert W_1^{(h)}\theta - W_1^{(h)}\theta' \rVert \lVert W_1^{(h)} \rVert \;\;(\because \psi' \text{ is } L_{\psi'}-\text{Lipschitz})\\
        & = L_{\psi'} \lVert W_2^{(h)} \rVert \lVert W_1^{(h)}\rVert \lVert \theta - \theta' \rVert \lVert W_1^{(h)} \rVert\\
        \implies \sigma_{\max}(J_{h(\theta)} - J_{h(\theta')}) & \leq \frac{1}{\sqrt{2\pi}}\sigma_{\max}(W_2^{(h)}) \cdot \sigma_{\max}^2(W_1^{(h)}) \lVert \theta - \theta' \rVert
    \end{align}
    where $L_{\psi'} = \frac{1}{\sqrt{2\pi}}$ for derivative of GeLU activation function. Using Lemma \ref{lem:warmup-jacobian-singular-whp} results for singular values of the random matrices $W_1^{(h)}$ and $W_2^{(h)}$, we get that w.p. $\geq 1 - 2e^{-\frac{d_1^{(h)}}{64}}$
    \begin{equation}
        \sigma_{\max}(J_{h(\theta)} - J_{h(\theta')}) \leq \frac{343(\sigma_1^{(h)})^2 \sigma_2^{(h)} (d_{1}^{(h)})^{3/2}}{64\sqrt{2\pi}} \lVert \theta - \theta' \rVert
    \end{equation}
\end{proof}

\begin{theorem}
    \label{th:warmup-main-claim}
    Consider two neural networks $h, g$ with parameters $\theta\in\mathbb{R}^{d_0^{(h)}}$ and $\phi\in\mathbb{R}^{d_0^{(g)}}$, respectively, defined as $h(\theta) = W_2^{(h)} \psi(W_1^{(h)}\theta)$ and $g(\phi) = W_2^{(g)} \psi(W_1^{(g)} \phi)$ where $W_k^{(h)} \sim \mathcal{N}(0,(\sigma_k^{(h)})^2 I_{d_{k}^{(h)} \times d_{k-1}^{(h)}})$ and $W_k^{(g)} \sim \mathcal{N}(0,(\sigma_k^{(g)})^2 I_{d_{k}^{(g)} \times d_{k-1}^{(g)}})$, $k\in\{1,2\}$ and $\psi$ is the GeLU activation function with $d_{1}^{(h)} \geq 256 d_{0}^{(h)}$, $d_{1}^{(h)} \geq 256 d_{2}^{(h)}$, $d_{1}^{(g)} \geq 256 d_{0}^{(g)}$, $d_{1}^{(g)} \geq 256 d_{2}^{(g)}$. For the $\varepsilon-\ell_2$-regularized bilinear min-max objective $f(\theta,\phi)$ as defined in Equation \ref{eq:warmup-min-max-objective} with the neural networks $h$ and $g$ defined above, alternating gradient-descent-ascent reaches the desired saddle point w.p. $\geq 1 - 4e^{-\frac{d_1^{(h)}}{64}} - 4e^{-\frac{d_1^{(g)}}{64}} - e^{-Cd_1^{(h)}} - e^{-Cd_1^{(g)}} $ if the initial parameters $(\theta_0,\phi_0)$ and standard deviations $\sigma_k^{(h)}$ and $\sigma_k^{(g)}$, $k\in\{1,2\}$ are chosen such that:
    \begin{align}
        \label{eq:warmup-main-claim}
        (\sigma_{1}^{(h)})^2 & < \frac{\pi}{4Cd_{1}^{(h)} \lVert \theta_0 \rVert^2} \\
        (\sigma_{1}^{(g)})^2 & < \frac{\pi}{4Cd_{1}^{(g)} \lVert \phi_0 \rVert^2} \\
        \frac{(\sigma_{1}^{(h)})^3 (\sigma_{2}^{(h)})^2}{\left( \frac{1}{2} - (\sigma_{1}^{(h)}) \lVert \theta_0 \rVert \sqrt{\frac{Cd_{1}^{(h)}}{\pi}}\right)^2} & < \frac{0.012\pi}{(\sqrt{2}\varepsilon L_f)\cdot (d_{1}^{(h)})^{2.5}} \\
        \frac{(\sigma_{1}^{(g)})^3 (\sigma_{2}^{(g)})^2}{\left( \frac{1}{2} - (\sigma_{1}^{(g)}) \lVert \phi_0 \rVert \sqrt{\frac{Cd_{1}^{(g)}}{\pi}}\right)^2} & < \frac{0.012\pi}{(\sqrt{2}\varepsilon L_f)\cdot (d_{1}^{(g)})^{2.5}} \\
        \frac{(\sigma_1^{(g)} \sigma_2^{(g)}) ((\sigma_1^{(h)})^2 \sigma_2^{(h)})}{\left( \frac{1}{2} - (\sigma_{1}^{(h)}) \lVert \theta_0 \rVert \sqrt{\frac{Cd_{1}^{(h)}}{\pi}}\right)^2} & < \frac{\pi}{1141692 L_f (1+\lambda) (d_{1}^{(h)})^{1.5}\sigma_{\max}(A)} \\
        \frac{((\sigma_1^{(g)})^3 \sigma_2^{(g)}) (\sigma_2^{(h)})}{\left( \frac{1}{2} - (\sigma_{1}^{(g)}) \lVert \phi_0 \rVert \sqrt{\frac{Cd_{1}^{(g)}}{\pi}}\right)^2} & < \frac{\pi}{1141692 L_f (1+\lambda) d_{1}^{(g)} \sqrt{d_{1}^{(h)}}\sigma_{\max}(A)} \\
        \frac{(\sigma_1^{(h)} \sigma_2^{(h)}) ((\sigma_1^{(g)})^2 \sigma_2^{(g)})}{\left( \frac{1}{2} - (\sigma_{1}^{(g)}) \lVert \phi_0 \rVert \sqrt{\frac{Cd_{1}^{(g)}}{\pi}}\right)^2} & < \frac{\pi}{1141692 L_f (d_{1}^{(g)})^{1.5}\sigma_{\max}(A)} \\
    \frac{((\sigma_1^{(h)})^3 \sigma_2^{(h)}) (\sigma_2^{(g)})}{\left( \frac{1}{2} - (\sigma_{1}^{(h)}) \lVert \theta_0 \rVert \sqrt{\frac{Cd_{1}^{(h)}}{\pi}}\right)^2} & < \frac{\pi}{1141692 L_f d_{1}^{(h)} \sqrt{d_{1}^{(g)}}\sigma_{\max}(A)}
    \end{align}
\end{theorem}
\begin{proof}
    Since $f(\theta,\phi)$ is $\varepsilon$-hidden-strongly-convex-strongly-concave, by Lemma \ref{lem:function-composition-pl-condition} it also satisfies the 2-sided PŁ-condition with ($\mu_\theta = \varepsilon\cdot \sigma_{\min}^2(J_{h(\theta)})$, $\mu_\phi = \varepsilon\cdot \sigma_{\min}^2(J_{g(\phi)})$) w.p. $\geq 1 - 2e^{-\frac{d_1}{64}} - e^{-Cd_1}$, we can utilise path-length bound as derived in Lemma \ref{lem:agda-dist-to-saddle} which leaves us with controlling the potential $P_0$ for ensuring convergence to the saddle point. Thus, continuing from \eqref{eq:P_0-bound-1}, we see that:
\begin{align}
    P_0 & \leq \lVert h(\theta_0) \rVert \cdot (\varepsilon L_f C_1 \sigma_{\max}(J_{h(\theta_0)}) + L_f (1+\lambda)C'_2 \sigma_{\max}(J_{g(\phi_0)}) \sigma_{\max}(A)) \nonumber \\ 
    & +  \lVert g(\phi_0) \rVert \cdot (L_f C_1 \sigma_{\max}(J_{h(\theta_0)})\sigma_{\max}(A) +\varepsilon (1+\lambda) C'_2)\sigma_{\max}(J_{g(\phi_0)}) \\
      & \leq (3.47\sigma_1^{(h)} \sigma_2^{(h)} d_1^{(h)}) \lVert h(\theta_0)\rVert \cdot (\underset{T_1}{\underbrace{\varepsilon L_f C_1}}) + (3.47\sigma_1^{(g)} \sigma_2^{(g)} d_1^{(g)}) \lVert h(\theta_0)\rVert \cdot (\underset{T_2}{\underbrace{L_f(1+\lambda)C'_2\sigma_{\max}(A)}}) \nonumber \\
      & + (3.47\sigma_1^{(h)} \sigma_2^{(h)} d_1^{(h)}) \cdot \lVert g(\phi_0) \rVert \cdot \underset{T_3}{\underbrace{(L_fC_1\sigma_{\max}(A))}} + (3.47\sigma_1^{(g)} \sigma_2^{(g)} d_1^{(g)}) \lVert g(\phi_0)\rVert \cdot (\underset{T_4}{\underbrace{\varepsilon (1+\lambda) C'_2}})\\
      & (\because \sigma_{\max}(J_{h(\theta_0)}) < 3.47\sigma_1^{(h)} \sigma_2^{(h)} d_1^{(h)}, \sigma_{\max} (J_{g(\phi_0)}) < 3.47\sigma_1^{(g)} \sigma_2^{(g)} d_1^{(g)}) \nonumber
\end{align}
Therefore, we want the following to hold true: 
\begin{enumerate}
    \item $(3.47\sigma_1^{(h)} \sigma_2^{(h)} d_1^{(h)}) \lVert h(\theta_0) \rVert \leq \frac{\kappa' R^2}{4T_1}$ 
    \item $(3.47\sigma_1^{(g)} \sigma_2^{(g)} d_1^{(g)}) \lVert h(\theta_0) \rVert \leq \frac{\kappa'' R^2}{4T_2}$ 
    \item $(3.47\sigma_1^{(h)} \sigma_2^{(h)} d_1^{(h)}) \lVert g(\phi_0) \rVert \leq \frac{\kappa' R^2}{4T_3}$ 
    \item $(3.47\sigma_1^{(g)} \sigma_2^{(g)} d_1^{(g)}) \lVert g(\phi_0) \rVert \leq \frac{\kappa'' R^2}{4T_4}$
\end{enumerate}
where $\kappa', \kappa'' \lesssim \kappa $. Specifically,
\begin{gather}
    \kappa = \frac{(1 - \sqrt{c})^2}{8\alpha'_1} = \frac{(1-c)^2}{8\alpha'_1(1+\sqrt{c})^2} \geq \frac{(1-c)^2}{32\alpha'_1}
\end{gather}
where we used the fact that $1 + \sqrt{c} \in [1,2]$. Furthermore, we use the observation that $\alpha'_1 \lesssim \frac{1}{\mu_\theta} + \frac{1}{\mu_\phi} \lesssim C \mu_{\theta}^{2.5}\mu_\phi^2$ ($C = 2/m^{5.5}$) since $\sigma_{\min}(J_{h(\theta)}), \sigma_{\min}(J_{g(\phi)}) \geq m > 0 $ for some $m$. This would yield
\begin{gather}
    \kappa \gtrsim \underset{\kappa'}{\underbrace{\frac{\mu_\theta \mu_{\phi}^{2}}{\mu_{\theta}^{2.5} \mu_{\phi}^{2}} = \frac{1}{\mu_{\theta}^{1.5}}}}
\end{gather}
Analogous reasoning by requiring $\alpha'_1 \lesssim \frac{1}{\mu_\theta} + \frac{1}{\mu_\phi} \lesssim C \mu_{\theta}\mu_\phi^{3.5}$ ($C = 2/m^{5.5}$), gives
\begin{equation}
    \kappa \gtrsim \underset{\kappa''}{\underbrace{\frac{\mu_\theta \mu_{\phi}^{2}}{\mu_{\theta} \mu_{\phi}^{3.5}} = \frac{1}{\mu_{\phi}^{1.5}}}} 
\end{equation}

Since $\lVert h(\theta_0) \rVert \leq \sigma_{\max}(W_2^{(h)}) \sigma_{\max}(\Psi(W_1^{(h)}\theta_0))$, using Lemma \ref{lem:warmup-jacobian-singular-whp} for maximum singular values of $W_2^{(h)}$ and $\Psi(W_1^{(h)}\theta)$, for ensuring 1.) holds, we will demand the following: $(3.47\sigma_1^{(h)} \sigma_2^{(h)} d_1^{(h)}) \cdot \left(\frac{7}{4}\sigma_2^{(h)} \sqrt{d_1^{(h)}}\right) \cdot 1.13 \leq \frac{\kappa R^2}{4T_1}$. This will yield the following sufficient condition on $\sigma_{1}^{(h)}$ and $\sigma_{2}^{(h)}$:
\begin{equation}
      \sigma_{1}^{(h)} (\sigma_{2}^{(h)})^2 \leq \frac{2\kappa' R^2}{54.9 \cdot (d_1^{(h)})^{3/2}\cdot T_1}
\end{equation}
By definition the radius $R \leq \frac{\mu_{\text{Jac}}^{(h)}}{2\beta_h}$. Substituting the lower bound for minimum singular value and Lipschitzness constant for Jacobian of network $h$ from Lemmas \ref{lem:warmup-jacobian-singular-whp}-\ref{lem:warmup-jacobian-smoothness}, we obtain:
\begin{equation}
    \frac{(\sigma_{1}^{(h)})^3 (\sigma_{2}^{(h)})^2}{\left( \frac{1}{2} - (\sigma_{1}^{(h)}) \lVert \theta_0 \rVert \sqrt{\frac{Cd_{1}^{(h)}}{\pi}}\right)^2} < \frac{0.012\pi\kappa'}{(\varepsilon L_f C_1)\cdot (d_{1}^{(h)})^{2.5}}
\end{equation}
Since $C_1 = \sqrt{\frac{2}{\mu_{\theta}^{3}}}$ and $\kappa' = \frac{1}{\mu_{\theta}^{1.5}}$, we get:
\begin{equation}
    \frac{(\sigma_{1}^{(h)})^3 (\sigma_{2}^{(h)})^2}{\left( \frac{1}{2} - (\sigma_{1}^{(h)}) \lVert \theta_0 \rVert \sqrt{\frac{Cd_{1}^{(h)}}{\pi}}\right)^2} < \frac{0.012\pi}{(\sqrt{2}\varepsilon L_f)\cdot (d_{1}^{(h)})^{2.5}}
\end{equation}
The same reasoning with $R \leq \frac{\mu_{\text{Jac}}^{(g)}}{2\beta_g}$ for ensuring 4.) holds true in case of $g(\phi_0)$ gives us a similar condition on $\sigma_{1}^{(g)}$ and $\sigma_{2}^{(g)}$:
\begin{equation}
      \frac{(\sigma_{1}^{(g)})^3 (\sigma_{2}^{(g)})^2}{\left( \frac{1}{2} - (\sigma_{1}^{(g)}) \lVert \phi_0 \rVert \sqrt{\frac{Cd_{1}^{(g)}}{\pi}}\right)^2} < \frac{0.012\pi}{(\sqrt{2}\varepsilon L_f)\cdot (d_{1}^{(g)})^{2.5}}
\end{equation}

For ensuring 2.), by Lemmas \ref{lem:warmup-jacobian-singular-whp}-\ref{lem:warmup-jacobian-smoothness} and using $R \leq \frac{\mu_{\text{Jac}}^{(h)}}{2\beta_h}$, we see that we need $(3.47\sigma_1^{(g)} \sigma_2^{(g)} d_1^{(g)}) \cdot \left(\frac{7}{4}\sigma_2^{(h)} \sqrt{d_1^{(h)}}\right) \cdot 1.13 \leq \frac{\kappa'' R^2}{4T_2}$ which yields the following sufficient condition:
\begin{align}
    (3.47\sigma_1^{(g)} \sigma_2^{(g)} d_1^{(g)}) \cdot \left(\frac{7}{4}\sigma_2^{(h)} \sqrt{d_1^{(h)}}\right) \cdot 1.13 & \leq \frac{\kappa'' R^2}{(4L_f(1+\lambda)C'_2\sigma_{\max}(A))} \\
    & \leq \frac{R^2}{4\sqrt{2}L_f(1+\lambda)\sigma_{\max}(A)} \\
    & \left(\because C'_2 = \sqrt{\frac{2}{\mu_{\phi}^{3}}}, \kappa'' = \frac{1}{\mu_{\phi}^{1.5}}\right) \\
    & = \frac{(\mu_{\text{Jac}}^{(h)})^2}{16\sqrt{2}L_f(1+\lambda)\sigma_{\max}(A)\beta_h^2} \\
    & \leq \frac{\left( \frac{1}{2} - (\sigma_{1}^{(h)}) \lVert \theta_0 \rVert \sqrt{\frac{Cd_{1}^{(h)}}{\pi}}\right)^2 \cdot \pi}{(343)^2 \sqrt{2}L_f(1+\lambda)\sigma_{\max}(A) (\sigma_{1}^{(h)})^2 d_{1}^{(h)}}\\
    & (\text{By Lemma }\ref{lem:warmup-jacobian-singular-whp}-\ref{lem:warmup-jacobian-smoothness}) \nonumber \\
    \implies \frac{(\sigma_1^{(g)} \sigma_2^{(g)}) ((\sigma_1^{(h)})^2 \sigma_2^{(h)})}{\left( \frac{1}{2} - (\sigma_{1}^{(h)}) \lVert \theta_0 \rVert \sqrt{\frac{Cd_{1}^{(h)}}{\pi}}\right)^2} & < \frac{\pi}{1141692 L_f (1+\lambda) (d_{1}^{(h)})^{1.5}\sigma_{\max}(A)}
\end{align} 
For ensuring 2.), if we were to use $R\leq \frac{\mu_{\text{Jac}}^{(g)}}{2\beta_g}$ instead, we would get the following condition:
\begin{align}
    \frac{((\sigma_1^{(g)})^3 \sigma_2^{(g)}) (\sigma_2^{(h)})}{\left( \frac{1}{2} - (\sigma_{1}^{(g)}) \lVert \phi_0 \rVert \sqrt{\frac{Cd_{1}^{(g)}}{\pi}}\right)^2} & < \frac{\pi}{1141692 L_f (1+\lambda) d_{1}^{(g)} \sqrt{d_{1}^{(h)}}\sigma_{\max}(A)}
\end{align}

Similarly, for ensuring 3.),  we see that we need $(3.47\sigma_1^{(h)} \sigma_2^{(h)} d_1^{(h)}) \cdot \left(\frac{7}{4}\sigma_2^{(g)} \sqrt{d_1^{(g)}}\right) \cdot 1.13 \leq \frac{\kappa R^2}{4T_3}$ which yields the following sufficient conditions when we use $R\leq \frac{\mu_{\text{Jac}}^{(g)}}{2\beta_g}$ and $R \leq \frac{\mu_{\text{Jac}}^{(h)}}{2\beta_h}$:
\begin{align}
    \frac{(\sigma_1^{(h)} \sigma_2^{(h)}) ((\sigma_1^{(g)})^2 \sigma_2^{(g)})}{\left( \frac{1}{2} - (\sigma_{1}^{(g)}) \lVert \phi_0 \rVert \sqrt{\frac{Cd_{1}^{(g)}}{\pi}}\right)^2} & < \frac{\pi}{1141692 L_f (d_{1}^{(g)})^{1.5}\sigma_{\max}(A)} \\
    \frac{((\sigma_1^{(h)})^3 \sigma_2^{(h)}) (\sigma_2^{(g)})}{\left( \frac{1}{2} - (\sigma_{1}^{(h)}) \lVert \theta_0 \rVert \sqrt{\frac{Cd_{1}^{(h)}}{\pi}}\right)^2} & < \frac{\pi}{1141692 L_f d_{1}^{(h)} \sqrt{d_{1}^{(g)}}\sigma_{\max}(A)}
\end{align}


This gives us sufficient conditions to instantiate the networks $h(\theta)$ and $g(\phi)$ analogous to conditions on random initializations of neural networks for training them.

% we are ensures that the iterates remain within the ball $B((\theta_0,\phi_0), R)$ around $(\theta_0,\phi_0)$ thereby ensuring that the Jacobian of the two neural networks remains non-singular within this ball. This will now help us check if $(\theta^*, \phi^*)$ reached by AltGDA is a saddle point by checking for first-order stationarity of $(\theta^*,\phi^*)$ (Definition \ref{def:sol-concept}). Towards this, by Lemma \ref{lem:warmup-jacobian-singular-whp} we know that the Jacobian of the two neural networks has non-zero minimum singular value w.p. $\geq 1 - 2e^{-\frac{d_1}{64}} - e^{-Cd_1}$ which would mean that we have $\nabla_\theta f(\theta^*,\phi^*) = J_{h(\theta^*)}^\top (Ag(\phi^*) + \varepsilon h(\theta^*)) = 0 $ and $\nabla_\phi f(\theta^*,\phi^*) = J_{g(\phi^*)}^\top( A^\top h(\theta^*) - \varepsilon g(\phi^*)) = 0$. That is, we must have $Ag(\phi^*) + \varepsilon h(\theta^*) = 0$ and $A^\top h(\theta^*) - \varepsilon g(\phi^*) = 0$. Note that $\nabla_z f(z^*, w^*) = Aw^* + \varepsilon z^*$ and $\nabla_w f(z^*, w^*) = A^\top z^* - \varepsilon w^*$ where $z^* = h(\theta^*)$ and $w^* = g(\phi^*)$. Thus, $(\theta^*, \phi^*)$ is a saddle point iff $\nabla_z f(z^*, w^*) = 0 = \nabla_w f(z^*, w^*)$. That is, $(\theta^*, \phi^*)$ is a saddle point of $f(\theta,\phi)$ iff $(z^*,w^*)$ is a stationary point of $f(z,w)$.
\end{proof}

\subsection{Main Result: Hidden-strongly-convex-hidden-strongly-concave min-max optimization with 1-hidden-layer neural networks}

\subsubsection{Estimating smoothness constant, minimum and maximum singular values of a two-layer neural network's Jacobian}

For ensuring the potential $P_0$ is small, we first estimate the lower and upper bounds for the singular values of the Jacobian along with its Lipschitz constant. This will allow us to find the right initialization $(\theta_0,\phi_0) $ which we will then use for determining the size of the neural networks needed for solving the min-max problem.

We follow \citeauthor{song2021subquadratic} \cite{song2021subquadratic} for computing the Lipschitzness constant and the high probability bounds for the lower and upper bounds of singular values of a 1-hidden-layer neural network for random Gaussian initializations. These quantities are first computed using a first-order Taylor-series approximation of the neural network Jacobian followed by using well-known results and tools from random matrix theory to obtain high probability concentration bounds for the relevant random variables at these random Gaussian initializations.

\begin{assumption}[Random Initialization]
    \label{ass:rand-init}
    We consider the following initialization scheme for a 1-hidden-layer neural network, $h$, as defined in Definition \ref{def:neural-net-def}:
    \begin{equation}
        (W_{1}^{(h)})_0 \sim \mathcal{N}(0, (\sigma_{1}^{(h)})^2 I) \quad \quad (W_{2}^{(h)})_0 \sim \mathcal{N}(0, (\sigma_{2}^{(h)})^2 I)
    \end{equation}
\end{assumption}

% \begin{lemma}[Lemma 3 in \cite{song2021subquadratic}]
% \label{lem:estim-jacobian}
%     Suppose that a two-layer neural network, $h$, as defined in Section \ref{sec:prelim}, satisfies Assumption \ref{ass:neural-net-def}. Then the neural network Jacobian has the following lower ($\mu_{\text{Jac}}^{(h)}$) and upper ($\nu_{\text{Jac}}^{(h)}$) bounds on its singular values and Lipschitz constant ($\beta_h$):
%     \begin{align}
%         \mu_{\text{Jac}}^{(h)} & = \sigma_{\min}(\psi((W_{1}^{(h)})_0 X)) \nonumber \\
%         \nu_{\text{Jac}}^{(h)} & = \dot \psi_{\max}\sigma_{\max}(X) \sigma_{\max}((W_{2}^{(h)})_0) +  \sigma_{\max}(\psi((W_{1}^{(h)})_0 X)) \\
%         \beta_h & = \sqrt{2}\sigma_{\max}(X)(\dot \psi_{\max} + \ddot \psi_{\max} \chi_{\max}) \nonumber
%     \end{align}
%     where $\chi_{\max} = \sup_V \sigma_{\max}(V)$.
% \end{lemma}
\begin{lemma}[Lemma 3 \& Appendix E.1--E.4 in \cite{song2021subquadratic}]
\label{lem:main-jacobian-singular-val-smoothness-whp}
    Suppose that a two-layer neural network, $h$, as defined in Definition \ref{def:neural-net-def}, satisfies Assumption \ref{ass:neural-net-act}. Suppose the activation function also satisfies $\tau^{r_1} |\psi(a)| \leq |\psi(\tau a)| \leq \tau^{r_2} |\psi(a)|$, respectively for all $a$, $0 < \tau < 1$,  and some constants $r_1, r_2$. Then the neural network Jacobian has the following lower bounds on its smallest singular value w.p. $\geq 1 - (p_1 + p_2)$:
    \begin{equation}
        \label{eq:jacobian-singular-lower-whp}
        \mu_{\text{Jac}}^{(h)} \geq (\sigma_1^{(h)})^{r_1} \sqrt{(1-\delta_1) \frac{c_t^2}{t!}d_{1}^{(h)}} \cdot \sigma_{\min}(X^{*t})
    \end{equation}
    Moreover, we also have the following upper bound on its largest singular value w.p. $\geq 1 - (p_1 + p_3 + p_4)$:
    \begin{align}
        \label{eq:jacobian-singular-higher-whp}
        \nu_{\text{Jac}}^{(h)} \lesssim \sigma_2^{(h)} & \dot \psi_{\max} \sigma_{\max}(X)\sqrt{d_{1}^{(h)}} + (\sigma_1^{(h)})^{r_1}\sqrt{(1+\delta_2)(c_1^2 + c_{\infty}^2) d_{1}^{(h)}} \sigma_{\max}(X) \nonumber \\
        &  + (\sigma_{1}^{(h)})^{r_2} |c_0| \sqrt{(1+\delta_2)d_{1}^{(h)}n}
    \end{align}
    where $\{c_i\}_i $ denote coefficient corresponding to ???, $\delta_j$'s are ???,.

    Also, the smoothness constant for the neural network can be computed as
    \begin{equation}
        \label{eq:jacobian-lipschitz}
        \beta_h = \sqrt{2}\sigma_{\max}(X)(\dot \psi_{\max} + \ddot \psi_{\max} \chi_{\max})
    \end{equation}
    where $\chi_{\max} = \sup_V \sigma_{\max}(V)$.
\end{lemma}



% \begin{remark}
%     This will give us conditions for what the initialization $(\sigma_1^{(h)}, \sigma_2^{(h)})$ and $(\sigma_1^{(g)}, \sigma_2^{(g)})$ should be.
% \end{remark}

\subsubsection{Combining everything so far}

We now utilize all the scaffolding built so far to obtain results about convergence to the saddle point using AltGDA for the the case of HSCSC games.

\begin{theorem}[HSCSC Games with AltGDA]
\label{th:main-agda-convergence}
Suppose there are two two-layer neural networks, $h_\theta$, $g_\phi$ as defined in Definition \ref{def:neural-net-def} which satisfy Assumption \ref{ass:neural-net-act}. Suppose the activation function $\psi$ also satisfies $\tau^{r_1} |\psi(a)| \leq |\psi(\tau a)| \leq \tau^{r_2} |\psi(a)|$, respectively for all $a$, $0 < \tau < 1$,  and some constants $r_1, r_2$. Suppose the network parameters $\theta_0$ and $\phi_0$ are randomly initialized as in Assumption \ref{ass:rand-init} with $(\sigma_1^{(h)}, \sigma_2^{(h)})$ and $(\sigma_1^{(g)}, \sigma_2^{(g)})$, respectively, which satisfy
\begin{equation}
    \sigma_1^{(h)} \sigma_2^{(h)} \lesssim \frac{1}{\sqrt{d_0^{(h)}d_{1}^{(h)}}}\quad \text{and} \quad \sigma_1^{(g)} \sigma_2^{(g)} \lesssim \frac{1}{\sqrt{d_0^{(g)}d_{1}^{(g)}}}
\end{equation}
and suppose that the hidden layer widths $d_1^{(h)}$ and $d_1^{(g)}$ for the two networks $h$ and $g$ satisfy 
\begin{align}
    d_1^{(h)} & = \widetilde{\Omega}\left( \xi(\mathcal{C}_\delta,t,\phi,\{c_i\}_{i\geq 0}) \frac{\sigma_{\max}(X)^6 n}{\sigma_{\min}(X^{*t})^4}\right) \\
    d_1^{(g)} & = \widetilde{\Omega}\left( \xi(\mathcal{C}_\delta,t,\phi,\{c_i\}_{i\geq 0}) \frac{\sigma_{\max}(X)^6 n}{\sigma_{\min}(X^{*t})^4}\right)
\end{align}
where $\mathcal{C}_\delta$ is a set of constants, $\xi$ and $\xi'$ are terms independent to $d$ and $n$, $t$ is a constant such that $n \simeq d^t$ and $X^{*t} \in \mathbb{R}^{d^t \times n}$ is derived from Khatri-Rao product with its $a$-th column defined as $\text{vec}(x_a \otimes \cdots x_a) \in \mathbb{R}^{d^t}$. Then Alternating Gradient-Descent-Ascent procedure with fixed step-sizes $\eta_h = , \eta_g =  $ for an HSCSC game with objective as defined in Equation \ref{eq:separable-min-max-objective} converges to the saddle point exponentially fast with probability at least $1 - \Lambda(\varepsilon, \psi,\xi,d_0^{(h)},d_0^{(g)},d_1^{(h)},d_1^{(g)},d_2^{(h)},d_2^{(g)})$.
\end{theorem}
\begin{proof}

For finding appropriate random initializations, based on Appendix E (E.5) in \citeauthor{song2021subquadratic} \cite{song2021subquadratic}, we can say for neural network, $F_\theta$, that w.p. $\geq 1 - (p_1 + p_5)$:
\begin{align}
    \label{eq:neural-net-output-upper-bound}
    \lVert F_{\theta_0}(X) \rVert & = \lVert (W_{2}^{(f)})_0 \psi((W_{1}^{(f)})_0 X) \rVert \nonumber \\
    & \leq \delta_3 \sigma_1^{(f)} \sigma_2^{(f)} \dot \psi_{\max} k_1 k_2 \cdot \sqrt{d_0^{(f)}\cdot d_{1}^{(f)} \cdot d_2^{(f)}} \cdot \sigma_{\max}(X) \log d_{1}^{(f)} \nonumber \\
    & \leq \delta_3 k_1 k_2 \sigma_{\max}(X) \;\;\left(\text{if } \sigma_1^{(f)}\sigma_2^{(f)} \lesssim \frac{1}{\dot \psi_{\max} \sqrt{d_0^{(f)}\cdot d_{1}^{(f)}\cdot d_2^{(f)}} \log d_{1}^{(f)}}\right)
\end{align}
where $p_5 = e^{-C\delta_3^2}$, and $\delta_3, k_1, k_2$ are constants independent of $d, m, n$.  Analogous reasoning gives a similar initialization condition for the neural network $G_\phi$.

Since our min-max objective $L_\mathcal{D}(F_\theta, G_\phi)$ is separable as defined in Equation \ref{eq:separable-min-max-objective}, we can start by rewriting the bilinear component $I_2^{\mathcal{D}}(F_\theta,G_\phi) = (F_\theta(\mathcal{D}_F))^\top A (G_\phi(\mathcal{D}_G))$. Now, using Assumption \ref{ass:grad-norm-strong-cvx}, we can compute the gradients for the min-max objective as follows given data $\mathcal{D} = (\mathcal{D}_F, \mathcal{D}_G)$:
\begin{align}
    \nabla_\theta L_\mathcal{D}(F_\theta, G_\phi) & = \nabla_\theta (I_1^{\mathcal{D}_F}(F_\theta) + I_2^{\mathcal{D}}(F_\theta,G_\phi))\\
    & = (J_{F_\theta}^{\mathcal{D}_F})^\top (\nabla_{z=F_\theta(\mathcal{D}_F)}I_1^{\mathcal{D}_F}(z)) + (J_{F_\theta}^{\mathcal{D}_F})^\top A G_\phi(\mathcal{D}_G) \\
    \nabla_\phi L_\mathcal{D}(F_\theta, G_\phi) & = \nabla_\phi (-I_3^{\mathcal{D}_G}(G_\phi) + I_2^{\mathcal{D}}(F_\theta,G_\phi))\\
    & = -(J_{G_\phi}^{\mathcal{D}_G})^\top (\nabla_{z=G_\phi(\mathcal{D}_G)}I_3^{\mathcal{D}_G}(z)) + (J_{G_\phi}^{\mathcal{D}_G})^\top A F_\theta(\mathcal{D}_F)
\end{align}
By Assumption \ref{ass:grad-norm-strong-cvx} on the gradient norm of strongly-convex functions, triangle inequality, and submultiplicativity of operator norm, we can say that the gradient norms of our separable min-max objective can be upper bounded as follows:
\begin{align}
    \lVert \nabla_\theta L_\mathcal{D}(F_\theta, G_\phi) \rVert & \leq
    \lVert (J_{F_\theta}^{\mathcal{D}_F})^\top \rVert \left( A_1^{(F)} \lVert F_{\theta_0}(\mathcal{D}_F) \rVert + A_2^{(F)} \text{diam}(\mathcal{Y}^{(F)}) + A_3^{(F)} \right) \nonumber \\ 
    & + \lVert (J_{F_\theta}^{\mathcal{D}_F})^\top \rVert \lVert A \rVert \lVert G_\phi(\mathcal{D}_G) \rVert \\
    \lVert \nabla_\phi L_\mathcal{D}(F_\theta, G_\phi) \rVert & \leq \lVert (J_{G_\phi}^{\mathcal{D}_G})^\top \rVert \left( A_1^{(G)} \lVert G_{\phi_0}(\mathcal{D}_G) \rVert + A_2^{(G)} \text{diam}(\mathcal{Y}^{(G)}) + A_3^{(G)} \right) \nonumber \\
    & + \lVert(J_{G_\phi}^{\mathcal{D}_G})^\top\rVert \lVert A \rVert \lVert F_\theta(\mathcal{D}_F) \rVert
\end{align}

Continuing from Equation \eqref{eq:P_0-upper-gradients}, we see that:
\begin{align}
    P_0 & \leq \underset{T_1}{\underbrace{C_1 \cdot(J_{F_{\theta_0}}^{\mathcal{D}_F})^\top \rVert \cdot \left( A_1^{(F)} \lVert F_{\theta_0}(\mathcal{D}_F) \rVert + A_2^{(F)} \text{diam}(\mathcal{Y}^{(F)}) + A_3^{(F)} \right)}} \nonumber \\ 
    & + \underset{T_2}{\underbrace{C_1 \cdot \lVert (J_{F_{\theta_0}}^{\mathcal{D}_F})^\top \rVert \lVert A \rVert \lVert G_{\phi_0}(\mathcal{D}_G) \rVert}} \nonumber\\
    & + \underset{T_3}{\underbrace{C_2 \cdot \lVert (J_{G_{\phi_0}}^{\mathcal{D}_G})^\top \rVert \cdot \left( A_1^{(G)} \lVert G_{\phi_0}(\mathcal{D}_G) \rVert + A_2^{(G)} \text{diam}(\mathcal{Y}^{(G)}) + A_3^{(G)} \right)}} \nonumber \\
    & + \underset{T_4}{\underbrace{C_2 \cdot \lVert(J_{G_{\phi_0}}^{\mathcal{D}_G})^\top\rVert \lVert A \rVert \lVert F_{\theta_0}(\mathcal{D}_F) \rVert}}
        % & \leq (\sigma_{\max}(V_0) \sigma_{\max}(\psi(W_0 X))) \cdot A_1 + 
        % (\sigma_{\max}(Q_0) \sigma_{\max}(\psi(R_0 X))) \cdot A_2 \nonumber \\
        % & +  A_3 \cdot (\sigma_{\max}(V_0) \sigma_{\max}(\psi(W_0 X)))^2 + A_4 \cdot (\sigma_{\max}(Q_0) \sigma_{\max}(\psi(R_0 X)))^2 \Big)
        % \implies P_0 & \lesssim (\sigma_2 \cdot \sqrt{m} \cdot \sqrt{(1+\delta_2)} \cdot \sigma_1^{r_2} \cdot (\sqrt{c_1^2 + c_\infty^2}\cdot m \cdot \sigma_{\max}(X) + \vert c_0\vert \sqrt{m n})) \cdot A_1 \nonumber\\ 
        % & + (\gamma_2 \cdot \sqrt{m} \cdot \sqrt{(1+\delta'_2)} \cdot \gamma_{1}^{r'_2} (\sqrt{s_{1}^{2} + s_\infty^2} \cdot m \cdot \sigma_{\max}(X) + \vert s_0\vert \sqrt{m n}))\cdot A_2 \nonumber \\
        % & + (\sigma_2 \cdot \sqrt{m} \cdot \sqrt{(1+\delta_2)} \cdot \sigma_1^{r_2} \cdot (\sqrt{c_1^2 + c_\infty^2}\cdot m \cdot \sigma_{\max}(X) + \vert c_0\vert \sqrt{m n}))^2 \cdot A_3 \nonumber\\
        % & + (\gamma_2 \cdot \sqrt{m} \cdot \sqrt{(1+\delta'_2)} \cdot \gamma_{1}^{r'_2} (\sqrt{s_{1}^{2} + s_\infty^2} \cdot m \cdot \sigma_{\max}(X) + \vert s_0\vert \sqrt{m n}))^2 \cdot A_4
\end{align}

In order to ensure $P_0 = \kappa R^2$ as per Equation \eqref{eq:P0-radius-bound} so that we stay within the ball $B((\theta_0,\phi_0), R)$ for the entire AltGDA trajectory thereby ensuring neural network Jacobians remain non-singular for both $F$ and $G$ for the entire trajectory, what we want is the following: 
\begin{enumerate}
    \item $T_1 \leq \frac{\kappa' R^2}{4}$
    \item $T_2 \leq \frac{\kappa' R^2}{4}$
    \item $T_3 \leq \frac{\kappa'' R^2}{4}$
    \item $T_4 \leq \frac{\kappa'' R^2}{4}$
\end{enumerate}
where $\kappa', \kappa'' \lesssim \kappa $. Specifically,
\begin{gather}
    \kappa = \frac{(1 - \sqrt{c})^2}{8\alpha'_1} = \frac{(1-c)^2}{8\alpha'_1(1+\sqrt{c})^2} \geq \frac{(1-c)^2}{32\alpha'_1}
\end{gather}
where we used the fact that $1 + \sqrt{c} \in [1,2]$. Furthermore, we use the observation that $\alpha'_1 \lesssim \frac{1}{\mu_\theta} + \frac{1}{\mu_\phi} \lesssim C \mu_{\theta}^{2.5}\mu_\phi^2$ ($C = 2/m^{5.5}$) since $\mu_{\text{Jac}}^{(F)}, \mu_{\text{Jac}}^{(G)} \geq m > 0 $ for some $m$ and $\mu_\theta \geq \mu_1 (\mu_{\text{Jac}}^{(F)})^2 $ and $\mu_\phi \geq \mu_2 \cdot(\mu_{\text{Jac}}^{(G)})^2$. This would yield
\begin{gather}
    \kappa \gtrsim \underset{\kappa'}{\underbrace{\frac{\mu_\theta \mu_{\phi}^{2}}{\mu_{\theta}^{2.5} \mu_{\phi}^{2}} = \frac{1}{\mu_{\theta}^{1.5}}}}
\end{gather}
Analogous reasoning by requiring $\alpha'_1 \lesssim \frac{1}{\mu_\theta} + \frac{1}{\mu_\phi} \lesssim C \mu_{\theta}\mu_\phi^{3.5}$ ($C = 2/m^{5.5}$), gives
\begin{equation}
    \kappa \gtrsim \underset{\kappa''}{\underbrace{\frac{\mu_\theta \mu_{\phi}^{2}}{\mu_{\theta} \mu_{\phi}^{3.5}} = \frac{1}{\mu_{\phi}^{1.5}}}} 
\end{equation}

Here, just like in Section \ref{subsec:warmup-safe-init}, we will define the ball radius $R$ as $R = \frac{\mu_{\text{Jac}}}{2\beta}$ with $\mu_{\text{Jac}} = \min\{\mu_{\text{Jac}}^{(F)}, \mu_{\text{Jac}}^{(G)}\}$ and $\beta = \max\{\beta_F,\beta_G\}$ where $\mu_{\text{Jac}}^{(F)}, \mu_{\text{Jac}}^{(G)}$ are lower bounds for the smallest singular value and $\beta_F$, $\beta_G$ are Lipschitz constant of the neural network Jacobian for networks $F_\theta$ and $G_\phi$, respectively. This radius $R$ is chosen so that if we can ensure that the Jacobian singular values are bounded away from zero and also bounded from above, then they continue to remain so within $\mathcal{B}((\theta_0,\phi_0), R)$ (Lemma 1 of \citeauthor{song2021subquadratic} \cite{song2021subquadratic}).
    % We can get the following bound on the initialization hyperparameters $\sigma_1, \sigma_2$ 
    % \begin{align}
    %     \sigma_1^{r_2} \sigma_2 < \frac{1}{C_{A_1}} \min\left( \frac{\kappa R^2}{4A_1}, \frac{\sqrt{\kappa} R}{2\sqrt{A_3}} \right) \\
    %     \sigma_1 \sigma_2 \lesssim \frac{1}{\dot \psi_{\max} \sqrt{d\cdot m\cdot d_h} \log m}
    % \end{align}
    % where $C_{A_1} = \sqrt{m(1+\delta_2)} \cdot (\sqrt{c_1^2 + c_\infty^2}\cdot m \cdot \sigma_{\max}(X) + \vert c_0\vert \sqrt{m n}))$. This can be simplified further if, say, we choose $\sigma_1 = 1$. In that case, we have the following initialization condition:
    % \begin{equation}
    %     \sigma_2 \lesssim \min\left( \frac{\kappa R^2}{4A_1 C_{A_1}}, \frac{\sqrt{\kappa} R}{2\sqrt{A_3} C_{A_1}}, \frac{1}{\dot \psi_{\max} \sqrt{dm} \log m} \right)
    % \end{equation}
     % and $(3\nu_\Phi/2)^2 \lVert g(\phi_0) \rVert^2 \leq \frac{\kappa R^2}{4A_4}$ % We can get the following bound on the initialization hyperparameters $\gamma_1, \gamma_2$ 
    % \begin{align}
    %     \gamma_1^{r_2} \gamma_2 < \frac{1}{C_{A_2}} \min\left( \frac{\kappa R^2}{4A_2}, \frac{\sqrt{\kappa} R}{2\sqrt{A_4}} \right) \\
    %     \gamma_1 \gamma_2 \lesssim \frac{1}{\dot \psi_{\max} \sqrt{d\cdot m\cdot d_g} \log m}
    % \end{align}
    % where $C_{A_1} = \sqrt{m(1+\delta'_2)} \cdot (\sqrt{s_1^2 + s_\infty^2}\cdot m \cdot \sigma_{\max}(X) + \vert s_0\vert \sqrt{m n}))$. This can be simplified further if, say, we choose $\gamma_1 = 1$. In that case, we have the following initialization condition:
    % \begin{equation}
    %     \gamma_2 \lesssim \min\left( \frac{\kappa R^2}{4A_2 C_{A_2}}, \frac{\sqrt{\kappa} R}{2\sqrt{A_4} C_{A_2}}, \frac{1}{\dot \psi_{\max} \sqrt{d\cdot m\cdot d_g} \log m} \right)
    % \end{equation}


% We also know from matrix norm properties that
% \begin{align*}
%     \lVert h(w_0) \rVert & = \lVert V_0 \psi(W_0 X)\rVert \nonumber \\ 
%     & \leq \sigma_{\max}(V_0) \sigma_{\max}(\psi(W_0 X)) \nonumber \\
%     & \lesssim \sigma_2 \cdot \sqrt{m} \cdot \sqrt{(1+\delta_2)} \cdot \sigma_1^{r_2} \cdot (\sqrt{c_1^2 + c_\infty^2}\cdot m \cdot \sigma_{\max}(X) + \vert c_0\vert \sqrt{m n})
% \end{align*}
% If we assume $\vert c_0 \vert$ to be sufficiently large such that $\vert c_0 \vert \sqrt{mn}$ becomes the dominant term for upper bound of $\lVert h(w_0) \rVert$, then a sufficient condition to ensure $\lVert h(w_0) \rVert \leq \min\left( \frac{\kappa R^2}{4A_1}, \frac{\sqrt{\kappa}R}{2\sqrt{A_3}}\right)$ will be:
% \begin{align}
%     \delta_3 k_1 k_2 \sigma_{\max}(X) & \lesssim \sigma_2 \cdot \sqrt{(1+\delta_2)} \cdot \sigma_1^{r_2} \cdot \vert c_0\vert \cdot m \cdot \sqrt{n} \nonumber \\
%     \implies m \gtrsim & \frac{\delta_3 k_1 k_2 \sigma_{\max}(X)}{\sigma_2 \cdot \sqrt{(1+\delta_2)} \cdot \sigma_1^{r_2} \cdot \vert c_0\vert \cdot \sqrt{n}} \\
%     \implies m & \gtrsim \xi(\{\delta_j\}_j, k_1, k_2, c_0, \phi, \sigma_1, \sigma_2) \cdot \frac{\sigma_{\max}(X)}{\sqrt{n}}
% \end{align}
% By Section 2.1 in \citeauthor{oymak2020toward} \cite{oymak2020toward}, we have $\sigma_{\max}(X) \simeq \sqrt{\frac{n}{d}}$. Then,
% \begin{align}
%     m & \gtrsim \xi(\{\delta_j\}_j, k_1, k_2, c_0, \phi, \sigma_1, \sigma_2) \cdot \frac{1}{\sqrt{d}} \\
%     \implies m \cdot d & \gtrsim \xi(\{\delta_j\}_j, k_1, k_2, c_0, \phi, \sigma_1, \sigma_2) \cdot \sqrt{d} \\
%     \implies m \cdot d & \gtrsim \xi(\{\delta_j\}_j, k_1, k_2, c_0, \phi, \sigma_1, \sigma_2) \cdot n^{1/4} \;\; (\because n \simeq d^2 \text{, typically}) \label{eq:overparam-bound-h}
% \end{align}

We will show arguments for the case of the `min' player (neural network $F_\theta$) here. Exactly the same arguments provide the analogous result for the `max' player (neural network $G_\phi$).

For ensuring (1.)--(4.), we will use the fact that $\sigma_{\max}(J_{F_{\theta_0}}^{\mathcal{D}_F}) \leq \nu_{\text{Jac}}^{(F)}$, $ \sigma_{\max}(J_{G_{\phi_0}}^{\mathcal{D}_G}) \leq \nu_{\text{Jac}}^{(G)}$, Lemma \ref{lem:main-jacobian-singular-val-smoothness-whp} for upper bounds on $\nu_{\text{Jac}}^{(F)}$, and $\nu_{\text{Jac}}^{(G)}$ and smoothness constants for two-layer neural networks along with the upper bounds on neural network outputs for $F$ and $G$ as derived above in Equation \eqref{eq:neural-net-output-upper-bound}.

Thus, a sufficient condition for ensuring 1.) would be as follows (assuming $|c_0|$ is sufficiently large s.t. $|c_0| \sqrt{(1+\delta_2)d_1^{(f)}n}$ becomes the dominating term in $\nu_{\text{Jac}}^{(F)}$): 
    \begin{gather}
        \underset{(LHS)}{\underbrace{C_1 \cdot \left(|c_0| \sqrt{(1+\delta_2)d_1^{(f)}n}\right) \cdot \left( A_1^{(F)} \delta_3 k_1 k_2 \sigma_{\max}(X) + A_2^{(F)} \text{diam}(\mathcal{Y}^{(F)}) + A_3^{(F)} \right)}}  \leq \frac{\kappa'}{4} \left(\frac{\mu_{\text{Jac}}^{(F)}}{2\beta_F}\right)^2 \nonumber\\
        \implies (LHS) \lesssim \frac{\kappa'}{16} \cdot \frac{(\sigma_{1}^{(f)})^{2 r_1}(1-\delta_1) (c_{t}^{2}/t!) d_1^{(f)} \sigma_{\min}^2(X^{*t})}{2(\sigma_{\max}(X))^{2} (\dot \psi_{\max} + \ddot \psi_{\max} \chi_{\max})^2} \;\;(\text{By Lemma }\ref{lem:main-jacobian-singular-val-smoothness-whp}) \\
        \implies d_1^{(f)} \gtrsim \frac{\left(C_1^2 |c_0|^2 (1+\delta_2)n \right) \cdot (32)^2(\sigma_{\max}(X))^{4} (\dot \psi_{\max} + \ddot \psi_{\max} \chi_{\max})^4 \cdot ( A_1^{(F)} \delta_3 k_1 k_2 \sigma_{\max}(X))^2}{(\kappa')^2 (\sigma_{1}^{(f)})^{2 + 2r_1}(1-\delta_1)^2 (c_{t}^{4}/(t!)^2)\sigma_{\min}^{4}(X^{*t})} \\
        \implies d_1^{(f)} \gtrsim \frac{\left(|c_0|^2 (1+\delta_2)n \right) \cdot (32)^2(\sigma_{\max}(X))^{4} (\dot \psi_{\max} + \ddot \psi_{\max} \chi_{\max})^4 \cdot ( A_1^{(F)} \delta_3 k_1 k_2 \sigma_{\max}(X))^2}{(\sigma_{1}^{(f)})^{2 + 2r_1}(1-\delta_1)^2 (c_{t}^{4}/(t!)^2)\sigma_{\min}^{4}(X^{*t})} \\
        \left(\because \kappa' = \frac{1}{\mu_{\theta}^{1.5}}, C_1 = \sqrt{\frac{2}{\mu_{\theta}^{3}}}\right) \\
        \implies d_1^{(f)} \gtrsim \xi(C_\delta,t, \psi, \{c_i\}_{i\geq0}) \frac{n \sigma_{\max}^6(X)}{\sigma_{\min}^{4}(X^{*t})}
        % \implies \delta_3 k_1 k_2 \sigma_{\max}(X) \sqrt{d_1^{(h)}n}  \lesssim \frac{\kappa}{16C_1} \cdot \frac{(\sigma_{1}^{(h)})^{2 r_1}(1-\delta_1) (c_{t}^{2}/t!) d_1^{(h)} \sigma_{\min}^2(X^{*t})}{2(\sigma_{\max}(X))^{2} (\dot \psi_{\max} + \ddot \phi_{\max} \chi_{\max})^2} \nonumber\\
        % \implies d_1^{(h)} \gtrsim \xi_1(\ldots) n \sigma_{\max}^{6}(X) \nonumber\\
        % \implies d_1^{(h)}  \gtrsim \xi_1(\ldots) \left(\frac{n}{d_0^{(h)}}\right)^3 n \nonumber\\
        % \implies d_1^{(h)} d_0^{(h)}  \gtrsim \xi_1(\ldots) n^{3} \;\;\left(\because t \geq 2, n \simeq (d_0^{(h)})^t, \sigma_{\max}(X) \simeq \sqrt{\frac{n}{d_0^{(h)}}}\right) \label{eq:deg-param-h-1}
    \end{gather}
where $\delta_4 = \max\{k_1, k_2\}$, $C_\delta = \{\delta_1,\delta_2,\delta_3,\delta_4\}$, and 
\[
    \xi(C_\delta,t, \psi, \{c_i\}_{i\geq0}) = \frac{\left(|c_0|^2 (1+\delta_2) \right) \cdot (32)^2( (\dot \psi_{\max} + \ddot \psi_{\max} \chi_{\max})^4 \cdot ( A_1^{(F)} \delta_3 k_1 k_2)^2}{(\sigma_{1}^{(f)})^{2 + 2r_1}(1-\delta_1)^2 (c_{t}^{4}/(t!)^2)}
\]
Here, along the lines of Section 2.1 in \citeauthor{oymak2020toward} \cite{oymak2020toward}, when we use the fact that $\sigma_{\max}(X) \simeq \sqrt{\frac{n}{d_0^{(f)}}}$ (since $\lVert x_i \rVert = 1$ for all rows $x_i$ of $X$), $\sigma_{\min}(X^{*t}) \simeq \sqrt{\frac{n}{(d_0^{(f)})^t}} \simeq 1$, and $n \simeq (d_0^{(f)})^t$ where $t \geq 2$, we get that:
\begin{equation}
    d_1^{(f)} = \tilde{\Omega}\left(\frac{n \cdot n^3}{(d_0^{(f)})^3 \cdot 1}\right) = \tilde{\Omega}\left( \frac{n^3}{d_0^{(f)}} \right)
\end{equation}

Thus, we have w.p. $\geq 1 - (p_1 + p_2 + p_3 + p_4 + p_5)$:
\begin{equation}
    \label{eq:deg-param-F-combined}
    d_1^{(f)} d_0^{(f)} = \tilde{\Omega}(n^3)
\end{equation}

Analogous reasoning for ensuring (3.) gives us w.p. $\geq 1 - $:
\begin{equation}
    d_1^{(g)} \gtrsim \xi(L_f, C'_\delta,t', \psi, \{c'_i\}_{i\geq0}) \frac{n \sigma_{\max}^6(X)}{\sigma_{\min}^{4}(X^{*t})}
\end{equation}
Use arguments from \citeauthor{oymak2020toward} \cite{oymak2020toward} above, we get a similar cubic overparameterization bound for the `max' player, $G_\phi$, as well:
\begin{equation}
    \label{eq:deg-param-g-combined}
    d_1^{(g)} d_0^{(g)} = \tilde{\Omega}(n^3)
\end{equation}




\end{proof}

\begin{remark}
    The proof above requires activation function to not be an odd function for ensuring $c_0 \neq 0$.    
\end{remark}


\subsubsection{Order analysis to determine amount of overparameterization ($t \geq 2$)}

\begin{lemma}[Cubic overparameterization for HSCSC games]
\label{lem:cubic-overparam}
    Suppose there are two 1-hidden-layer neural networks, $h$ and $g$, as defined and randomly initialized in Theorem \ref{th:main-agda-convergence} and suppose their Jacobians satisfy the high probability bounds on lower and upper bounds on singular values as in Lemma \ref{lem:estim-jacobian-whp}. In order to solve the HSCSC game and reach the saddle point $(\theta^*, \phi^*)$, one needs 
    \begin{gather}
        d_0^{(h)} d_1^{(h)} \gtrsim n^3 \\
        d_0^{(g)} d_1^{(g)} \gtrsim n^3 \\
    \end{gather}
    degree of overparameterization.
\end{lemma}


==> prelims.tex <==
% !TEX root = ./neurips_2025.tex

\section{Preliminaries}
\label{sec:prelim}
%\textbf{Preliminaries: Smoothness and Lipschitz Properties}
We begin by introducing the standard notions of smoothness and Lipschitz continuity that will be used throughout this work. All norms are taken to be the Euclidean (\(\ell_2\)) norm unless otherwise stated.
\paragraph{Lipschitz Continuity, Smoothness, and Strong Convexity}
Let \( f: \mathbb{R}^d \to \mathbb{R} \) be a differentiable function. We say that \(f\) is \(L_f\)-Lipschitz continuous and \(L_{\nabla f}\)-smooth if there exist constants \(L_f, L_{\nabla f} > 0\) such that
\[
|f(u) - f(v)| \leq L_f \|u - v\|, \quad \|\nabla f(u) - \nabla f(v)\| \leq L_{\nabla f} \|u - v\|, \quad \forall u,v \in \mathbb{R}^d.
\]
Moreover, \(f\) is \(\mu\)-strongly convex if there exists \(\mu > 0\) such that
\[
f(v) \geq f(u) + \langle \nabla f(u), v - u \rangle + \frac{\mu}{2} \|v - u\|^2, \quad \forall u, v \in \mathbb{R}^d.
\]
Similarly, for a parametrized mapping \(M_\theta(x): \mathbb{R}^{d_0} \to \mathbb{R}^{d_2}\) with parameters \(\theta \in \mathbb{R}^M\), we say \(M_\theta\) is \(\beta_M\)-smooth (w.r.t. \(\theta\)) at fixed input \(x\) if
\[
\sigma_{\max}\left( \nabla_\theta M_\theta(x) - \nabla_\theta M_{\theta'}(x) \right) \leq \beta_M \|\theta - \theta'\|, \quad \forall \theta, \theta' \in \mathbb{R}^M,
\]
where \(\sigma_{\max}(\cdot)\) denotes the largest singular value and \(\nabla_\theta M_\theta(x)\) is the Jacobian of \(M_\theta(x)\) with respect to \(\theta\).
\paragraph{Finite-Sample Parametrized Min-Max Setting}
Then, we unroll the general hidden convex–concave model of \eqref{eq:main-problem} to the finite-sample empirical risk minimization (ERM) setting, assuming access to a (possibly labeled) dataset \(\data = \{(x_i, y_i)\}_{i=1}^n\) of size \(n\). Formally, we consider the following optimization problem:
\begin{equation}\min_{\theta \in \mathbb{R}^{d_{\text{input}}^\opmin}} \max_{\phi \in \mathbb{R}^{d_{\text{input}}^\opmax}} \loss_\data(\opmin_\theta, \opmax_\phi):=
I_1^{\data_\opmin}(\opmin_\theta) + I_2^{(\data_\opmin,\data_\opmax)}(\opmin_\theta, \opmax_\phi) - I_3^{\data_\opmax}(\opmax_\phi),
\label{eq:min-max-struct} \tag{$\diamond$}
\end{equation}
where the mappings \(\opmin_\theta: \data_\opmin \to \strategyspace_\opmin\) and \(\opmax_\phi: \data_\opmax \to \strategyspace_\opmax\) are smooth functions parametrized by \(\theta\) and \(\phi\) (e.g., neural networks).
The individual components and the bilinear coupling expand as:
\begin{itemize}[nosep,leftmargin=*]
    \item \( I_1^{\data_\opmin}(\opmin_\theta) = \sum_{i \in [|\data_\opmin|]} \ell_i(y_i, \opmin_\theta(x_i))\),  \( I_3^{\data_\opmax}(\opmax_\phi) = \sum_{j \in [|\data_\opmax|]} \ell_j(y_j, \opmax_\phi(x_j))\),
    \item \( I_2^{(\data_\opmin,\data_\opmax)}(\opmin_\theta, \opmax_\phi) = \sum_{i \in [|\data_\opmin|]} \sum_{j \in [|\data_\opmax|]} \opmin_\theta(x_i)^\top A(x_i,x_j,y_i,y_j) \opmax_\phi(x_j)\),
\end{itemize}
where for each sample pair \(e_{ij}(x_i, x_j, y_i, y_j)\), the coupling matrix \(A(x_i,x_j,y_i,y_j) \in \mathbb{R}^{|\strategyspace_\opmin| \times |\strategyspace_\opmax|}\) encodes interactions between players.
\begin{assumption}
\begin{itemize}[nosep,leftmargin=*]
    \item Each \(\ell_i(y_i, \opmin_\theta(x_i))\) and \(\ell_j(y_j, \opmax_\phi(x_j))\) is a smooth function of \(\theta\) and \(\phi\), respectively.
    \item Each \(\ell_i\) (resp. \(\ell_j\)) is strongly convex with respect to \(\opmin_\theta(x_i)\) (resp. \(\opmax_\phi(x_j)\)).
\end{itemize}
\end{assumption}

\begin{assumption}[Gradient norm of strongly-convex objective]
\label{ass:grad-norm-strong-cvx}
Keeping parameters $\phi$ corresponding to the max player fixed, we have by assumption above that $f(\cdot,\phi)$ is $\mu_\theta$-hidden-strongly-convex. That is, $f(\cdot, \phi)$ is strongly-convex in $h(\cdot)$ for some (potentially non-linear; think of it as the neural network function for our case) function $h$. Re-writing this objective in the commonly used notation as a strongly-convex loss function $\mathcal{\ell}(\cdot,h_\theta(\cdot))$ for a given labelled pair of training data $(x, y)$, we note for a fixed $\phi$ that
\begin{equation}
    \mathcal{L}_h(\theta) = f(\theta,\phi) = \ell(y, h_\theta(x))
\end{equation}
Therefore, the norm of the gradient of $f(\theta,\phi)$ w.r.t. $\theta$ (for a given, fixed $\phi$) can be calculated using chain rule and Cauchy-Schwarz inequality as:
\begin{gather}
    \nabla_\theta \mathcal{L}_h(\theta) = \nabla_\theta f(\theta,\phi) =  \left(\frac{\partial h_\theta(x)}{\partial \theta}\right)^\top\nabla_h \ell(y, h)\\
    \implies \lVert \nabla_\theta \mathcal{L}_h(\theta) \rVert = \lVert \nabla_\theta f(\theta,\phi) \rVert \leq \left(\left\lVert \frac{\partial h_\theta(x)}{\partial \theta} \right\rVert \right) \cdot \lVert \nabla_h \ell(y,h)\rVert
\end{gather}
For commonly-used strongly-convex loss functions such as MSE, logistic loss, squared hinge loss and cross-entropy with $\ell_2$-regularization, we know that
\begin{equation}
    \lVert \nabla_h \ell(y,h)\rVert \leq A_1 \lVert h \rVert + A_2 \text{diam}(\mathcal{Y}) + A_3
\end{equation}
where $A_1$, $A_2$ and $A_3$ are constants dependent on the loss function and diam$(\mathcal{Y})$ denotes diameter of the label space $\mathcal{Y}$. Therefore, we can bound the gradient norm of the strongly-convex objective w.r.t. to the parameters as follows:
\begin{equation}
    \lVert \nabla_\theta \mathcal{L}_h(\theta) \rVert = \lVert \nabla_\theta f(\theta,\phi) \rVert \leq \left(\left\lVert \frac{\partial h_\theta(x)}{\partial \theta} \right\rVert \right) \cdot ( A_1 \lVert h_\theta(x) \rVert + A_2 \text{diam}(\mathcal{Y}) + A_3)
\end{equation}

\begin{assumption}[Gradient norm of strongly-convex objective]
\label{ass:grad-norm-strong-cvx}
Keeping parameters $\phi$ corresponding to the max player fixed, we have by assumption above that $f(\cdot,\phi)$ is $\mu_\theta$-hidden-strongly-convex. That is, $f(\cdot, \phi)$ is strongly-convex in $h(\cdot)$ for some (potentially non-linear; think of it as the neural network function for our case) function $h$. Re-writing this objective in the commonly used notation as a strongly-convex loss function $\mathcal{\ell}(\cdot,h_\theta(\cdot))$ for a given labelled pair of training data $(x, y)$, we note for a fixed $\phi$ that
\begin{equation}
    \mathcal{L}_h(\theta) = f(\theta,\phi) = \ell(y, h_\theta(x))
\end{equation}
Therefore, the norm of the gradient of $f(\theta,\phi)$ w.r.t. $\theta$ (for a given, fixed $\phi$) can be calculated using chain rule and Cauchy-Schwarz inequality as:
\begin{gather}
    \nabla_\theta \mathcal{L}_h(\theta) = \nabla_\theta f(\theta,\phi) =  \left(\frac{\partial h_\theta(x)}{\partial \theta}\right)^\top\nabla_h \ell(y, h)\\
    \implies \lVert \nabla_\theta \mathcal{L}_h(\theta) \rVert = \lVert \nabla_\theta f(\theta,\phi) \rVert \leq \left(\left\lVert \frac{\partial h_\theta(x)}{\partial \theta} \right\rVert \right) \cdot \lVert \nabla_h \ell(y,h)\rVert
\end{gather}
For commonly-used strongly-convex loss functions such as MSE, logistic loss, squared hinge loss and cross-entropy with $\ell_2$-regularization, we know that
\begin{equation}
    \lVert \nabla_h \ell(y,h)\rVert \leq A_1 \lVert h \rVert + A_2 \text{diam}(\mathcal{Y}) + A_3
\end{equation}
where $A_1$, $A_2$ and $A_3$ are constants dependent on the loss function and diam$(\mathcal{Y})$ denotes diameter of the label space $\mathcal{Y}$. Therefore, we can bound the gradient norm of the strongly-convex objective w.r.t. to the parameters as follows:
\begin{equation}
    \lVert \nabla_\theta \mathcal{L}_h(\theta) \rVert = \lVert \nabla_\theta f(\theta,\phi) \rVert \leq \left(\left\lVert \frac{\partial h_\theta(x)}{\partial \theta} \right\rVert \right) \cdot ( A_1 \lVert h_\theta(x) \rVert + A_2 \text{diam}(\mathcal{Y}) + A_3)
\end{equation}
\end{assumption}


Thus, \(I_1\) and \(I_3\) induce hidden strongly-convex and strongly-concave structures through the neural network mappings, while $I_2$ induce merely hidden convex-concave additional structure. It is straightforward to verify that under these assumptions, the min-max objective \eqref{eq:min-max-struct} defines a \((L_{\loss}, L_{\nabla\loss})\)-smooth and \((\mu_\theta, \mu_\phi)\)-hidden strongly convex–strongly concave problem, where the parameters depend on the properties of \(\{\ell_i\}\), \(\{A(x_i,x_j,y_i,y_j)\}\), and the smoothness of the mappings \(\opmin_\theta\) and \(\opmax_\phi\).Translating the known reductions from hidden strong convexity to PL-type conditions, we obtain:

\begin{fact}[Reduction to Two-Sided PL Condition, \parencite{fatkhullin2023stochastic, dorazio2025solving}]
\label{lem:function-composition-pl-condition}
The loss function \(\loss_\data\) satisfies a two-sided PL condition with parameters \(\mu_\theta \sigma_{\min}^2(\nabla_\theta \opmin_\theta)\) and \(\mu_\phi \sigma_{\min}^2(\nabla_\phi \opmax_\phi)\), where \(\sigma_{\min}(\cdot)\) denotes the smallest singular value of the corresponding Jacobians.
\end{fact}

\paragraph{Solution Concept}

What \underline{solution concepts} are we looking at? Let's first define the notion of global optima for our min-max problem:
\begin{definition}[Global Optima]
\label{def:sol-concept}We define three equivalent notions of optimality:
\begin{enumerate}
    \item $(\theta^*, \phi^*)$ is a global min-max point, if for any $(\theta,\phi)$: $f(\theta^*, \phi) \leq f(\theta^*, \phi^*) \leq \max_{\phi'} f(\theta,\phi')$
    \item $(\theta^*, \phi^*)$ is a saddle point, if for any $(\theta,\phi)$: $f(\theta^*, y) \leq f(\theta^*, \phi^*) \leq f(x, \phi^*)$
    \item $(\theta^*, \phi^*)$ is a stationary point, if for any $(\theta,\phi)$: $\nabla_{\theta} f(\theta^*, \phi^*) = \nabla_{\phi} f(\theta^*, \phi^*) = 0 $.
\end{enumerate}
\end{definition}
It's well known that these three notions of optimality are not necessarily equivalent for an arbitrary nonconvex-nonconcave min-max problems. It's also true that a saddle point or global min-max point may not always exist for min-max problems. So, we assume that a saddle point always exists in our work.

\begin{assumption}[Existence of saddle points]
    \label{ass:saddle-exist}
    The objective function has at least one saddle point. Moreover, we also assume that for any fixed $\phi$, $\min_{\theta\in \mathbb{R}^{m}}f(\theta,\phi)$ has a non-empty solution set and a finite optimal value. Similarly, for any fixed $\theta$, $\max_{\phi\in \mathbb{R}^{n}}f(\theta, \phi)$ has a non-empty solution set and a finite optimal value.
\end{assumption}

\begin{lemma}[Lemma 2.1 in \cite{yang2020global}] If the objective function $f$ satisfies two-sided PŁ-condition, then all the three notions of global optimality are equivalent for our min-max problem:
    \[
    \text{(saddle point)} \iff \text{(global min-max)} \iff \text{(stationary point)}
    \]
\end{lemma}




%Συνεχίζοντας κάνοντας εξειδικευοντας το model of \ref{?} following the finite sample ERM mode: υποθετοντας οτι ενα ((possible)labelled pairs of training data ) dataset D:\{(x,y)\}_{1..} of size $n$. (Γραψε το οπως το λενε στο neurips)
%\begin{equation}
%\opmax_\phi I_1^{\data_\opmin}(\opmin_\theta) + I_2^{(\data_\opmin,\data_\opmax)}(\opmin_\theta, \opmax_\phi) - I_3^{\data_{\opmax_\phi}}(\opmax_\phi),
%\label{eq:min-max-struct} \tag{?diamodn}
%\end{equation}
%where $\opmin_\theta: \data_\opmin \to \strategyspace_\opmin$ and $\opmax_\phi: \data_\opmax \to \strategyspace_\opmax$ are smooth mappings parameterized by $\theta$ and $\phi$ (e.g., neural network weights).
%We unroll the individual components and the bilinear coupling have that 
%\item I_1^{\data_\opmin}(\opmin_\theta)=\sum_{i\in [|\data_\opmin|]} \ell_i(y_i, \opmin_\theta(x_i))
%\item I_3^{\data_\opmax}(\opmax_\phi)=\sum_{j\in [|\data_\opmax|]} \ell_j(y_j, \opmax_\phi(x_j))
%\item I_2^{(\data_\opmin,\data_\opmax)}(\opmin_\theta, \opmax_\phi)(\opmin_\theta, \opmax_\phi)=\sum_{i\in [|\data_\opmin|]}\sum_{j\in [|\data_\opmax|]}  \opmin_\theta(x_i)^\top A(x_i,x_j,y_i,y_j)\opmax_\phi(x_j)
%where for a fixed element $elem:=(x_i,x_j,y_i,yJ)$ in dataset \data=(\data_\opmin,\data_\opmax) we have $A_ij=A(x_i,x_j,y_i,y_j)$ is an array of |\strategyspace_\opmin|\times|\strategyspace_\opmax| and 
%\ell_i(y_i, \opmin_\theta(x_i)),\ell_j(\phi)=\ell_j(y_j, \opmax_\phi(x_j)) are smooth function with respect to \theta (\phi) and strongly-convex function with respect to $\opmax_\theta$ (\opmin_\phi). And hence
%Hidden strongly-convex function with respect to $\theta$ (\phi). It is easy to check that under this model properties \eqref{eq:min-max-struct} is a ($L_{\loss},L_{\nabla\loss}$)-smooth $(\mu_\theta, \mu_\phi)$-hidden strongly-convex strongly-concave min-max problem for the induced by \ell_i,A_ij (\mu_\theta) with some modulus. Then, Translating the reduction hidden strong-convexity [Proposition 2 in \cite{fatkhullin2023stochastic}, Proposition 4.1 in \cite{dorazio2025solving}] to PL-condition to our setting
%
%\begin{fact}[Proposition 2 in \cite{fatkhullin2023stochastic}, Proposition 4.1 in \cite{dorazio2025solving}]
%    \label{lem:function-composition-pl-condition}
%    Loss L_\data satisfies  $\mu_\theta\sigma_{\min}^{2} (\nabla_\theta \ompin_\theta,\mu_\phi\sigma_{\min}^{2} (\nabla_\phi \ompax_\phi)$-twPŁ condition, where let $\sigma_{\min}$ be a lower bound on the singular values of {φτιαχτο } $J_{h(\theta)}=\frac{\partial h(\theta)}{\partial\theta}$. .
%\end{fact}

%%%
%%%
%%%\begin{assumption}
%%%\label{ass:min-max-obj-assumptions}
%%%The min-max objective function $f(\theta,\phi) $ is $(\mu_\theta, \mu_\phi)$-hidden-strongly-convex-hidden-strongly-concave, is $L_{f}$-Lipschitz and has $L_{f,grad}$-Lipschitz gradients.
%%%\end{assumption}







\begin{equation}
\min_{\theta \in \mathbb{R}^{d_{\text{input}}^h}} \max_{\phi \in \mathbb{R}^{d_{\text{input}}^g}} \loss_\data(\opmin_\theta, \opmax_\phi), \tag{$\prod$}
\end{equation}

While our results extend beyond, we focus on well-studied \cite{yuan2023optimal} \emph{separable} latent minmax objectives of the form
\[
\loss_\data(\opmin, \opmax) = I_1^{\data_\opmin}(\opmin) + I_2^{\data}(\opmin, \opmax) - I_3^{\data_\opmax}(\opmax),
\]


\clearpage

%%
%%\begin{definition}[Lipschitz Continuity and Smoothness]
%%\label{def:lipschitz-smoothness}
%%Let \( f: \mathbb{R}^d \to \mathbb{R} \) be a differentiable function. We say that:
%%\begin{itemize}
%%    \item \(f\) is \(L_f\)-Lipschitz if there exists a constant \(L_f > 0\) such that
%%    \[
%%    |f(u) - f(v)| \leq L_f \|u - v\|, \quad \forall u,v \in \mathbb{R}^d.
%%    \]
%%    
%%    \item \(f\) is \(L_{\nabla f}\)-smooth (i.e., has \(L_{\nabla f}\)-Lipschitz gradients) if there exists a constant \(L_{\nabla f} > 0\) such that
%%    \[
%%    \|\nabla f(u) - \nabla f(v)\| \leq L_{\nabla f} \|u - v\|, \quad \forall u,v \in \mathbb{R}^d.
%%    \]
%%\end{itemize}
%%Similarly, for a parametrized mapping \( M_\theta(x): \mathbb{R}^{d_0} \to \mathbb{R}^{d_2} \) depending on parameters \(\theta \in \mathbb{R}^M\), we say that \(M_\theta\) is \(\beta_M\)-smooth with respect to \(\theta\) at fixed input \(x\) if
%%\[
%%\sigma_{\max}\left( \nabla_\theta M_\theta(x) - \nabla_\theta M_{\theta'}(x) \right) \leq \beta_M \|\theta - \theta'\|, \quad \forall \theta, \theta' \in \mathbb{R}^M,
%%\]
%%where \(\sigma_{\max}(\cdot)\) denotes the largest singular value, and \(\nabla_\theta M_\theta(x)\) is the Jacobian of \(M_\theta(x)\) with respect to \(\theta\).
%%\end{definition}
%%
%%
%%\begin{definition}[Lipschitz Continuity and Smoothness]
%%\label{def:lipschitz-smoothness}
%%Let \( f: \mathbb{R}^d \to \mathbb{R} \) be a differentiable function. Then \(f\) is called \(L_f\)-Lipschitz (\(L_{\nabla f}\)-smooth) if there exists a constant \(L_f > 0\) (\(L_{\nabla f} > 0\)) such that
%%    \[
%%    |f(u) - f(v)| \leq L_f \|u - v\| \&    \|\nabla f(u) - \nabla f(v)\| \leq L_{\nabla f} \|u - v\|, \quad \forall u,v \in \mathbb{R}^d.
%%    \]
%%Similarly, for a parametrized mapping \( M_\theta(x): \mathbb{R}^{d_0} \to \mathbb{R}^{d_2} \) depending on parameters \(\theta \in \mathbb{R}^{M}\), we say that \(M_\theta\) is \(\beta_M\)-smooth with respect to \(\theta\) at fixed input \(x\) if
%%    \[
%%    \sigma_{\max}\left( \nabla_\theta M_\theta(x) - \nabla_\theta M_{\theta'}(x) \right) \leq \beta_M \|\theta - \theta'\|, \quad \forall \theta, \theta' \in \mathbb{R}^{M},
%%    \]
%%    where \(\sigma_{\max}(\cdot)\) denotes the largest singular value and $\nabla_\theta M_\theta(x)$ is Jacobian over theta.
%%\end{definition}
%%
%%
%%\begin{definition}[Smoothness of Scalar-Valued Functions]
%%\label{def:smooth-scalar}
%%A function \( f: \mathbb{R}^{d} \to \mathbb{R} \) is said to be \(\beta_f\)-smooth if it is differentiable and there exists a constant \(\beta_f > 0\) such that
%%\[
%%\|\nabla f(u) - \nabla f(v)\| \leq \beta_f \|u - v\|, \quad \forall u,v \in \mathbb{R}^d.
%%\]
%%\end{definition}
%%
%%\begin{definition}[Smoothness of Parametrized Mappings]
%%\label{def:smooth-param-map}
%%Let \( M_\theta(x): \mathbb{R}^{d_0} \to \mathbb{R}^{d_2} \) denote a mapping parametrized by \(\theta \in \mathbb{R}^{d_1}\).
%%We say that \(M\) is \(\beta_M\)-smooth with respect to \(\theta\) at fixed input \(x\) if
%%\[
%%\sigma_{\max}\left( \nabla_\theta M_\theta(x) - \nabla_\theta M_{\theta'}(x) \right) \leq \beta_M \|\theta - \theta'\|, \quad \forall \theta, \theta' \in \mathbb{R}^{d_1},
%%\]
%%where \(\sigma_{\max}(\cdot)\) denotes the largest singular value.
%%\end{definition}
%%
%%\begin{definition}[Lipschitz Continuity and Lipschitz Gradients]
%%\label{def:lip-func-lip-grad}
%%Let \(f: \mathbb{R}^{d_1} \times \mathbb{R}^{d_2} \to \mathbb{R}\) be a scalar-valued function.
%%\begin{itemize}
%%    \item \(f\) is \(L_f\)-Lipschitz if there exists \(L_f > 0\) such that
%%    \[
%%    |f(\theta,\phi) - f(\theta',\phi')| \leq L_f \left( \|\theta - \theta'\| + \|\phi - \phi'\| \right), \quad \forall \theta,\theta',\phi,\phi'.
%%    \]
%%    \item \(f\) has \(L_{\nabla f}\)-Lipschitz gradients if there exists \(L_{\nabla f} > 0\) such that
%%    \[
%%    \max \left\{ \|\nabla_\theta f(\theta,\phi) - \nabla_\theta f(\theta',\phi')\|,\, \|\nabla_\phi f(\theta,\phi) - \nabla_\phi f(\theta',\phi')\| \right\} \leq L_{\nabla f} \left( \|\theta - \theta'\| + \|\phi - \phi'\| \right),
%%    \]
%%    for all \(\theta,\theta',\phi,\phi'\).
%%\end{itemize}
%%\end{definition}
%%
%%
%%%Ξεκινάμε με τους ορισμούς οf smoothness ως προς την \ell_2 norm για μια συνάρτηση fun(p) : R^{dim_p }\to R και ενος parametrized for a fixed x M(\theta)=Map_\theta(x):R^{dim_1 }\to R^{dim_2 }
%%
%%\begin{definition}(Smoothness of neural network)
%%\label{def:smooth-neural-net}
%% Let $\beta_h > 0$. A neural network $h: \mathbb{R}^{d_{0}^{(h)}} \to \mathbb{R}^{d_{2}^{(h)}}$ is $\beta_h$-smooth, if for all $u,v \in \mathbb{R}^{d_{0}^{(h)}}$, we have 
%% \begin{equation}
%%     \label{eq:neural-net-smooth-def}
%%        \sigma_{\max}(\nabla h(u) - \nabla h(v)) \leq \beta_h \lVert u - v \rVert
%% \end{equation}
%%\end{definition}
%%
%% 
%%
%%\begin{definition}[Lipschitz function, Lipschitz gradients]
%%\label{def:lip-func-lip-grad}
%%A function $f$ is said to $L_f$-Lipschitz if there exists a positive constant $L_f > 0 $ such that
%%\begin{equation}
%%    \max \{ |f(\theta, \phi) - f(\theta, \phi')|, |f(\theta, \phi) - f(\theta', \phi)| \} \leq L_f (\lVert \theta - \theta' \rVert + \lVert \phi - \phi' \rVert) \;\forall \theta,\theta',\phi,\phi'.
%%\end{equation}
%%And the function $f$ is said to have $L_{f,grad}$-Lipschitz gradients if there exists a positive constant $ L_{f,grad} > 0 $ such that 
%%\begin{equation}
%%    \max \{ \lVert \nabla_{\phi}f(\theta, \phi) - \nabla_{\phi}f(\theta, \phi)\rVert, \lVert \nabla_{\theta}f(\theta, \phi) - \nabla_{\theta}f(\theta', \phi')\rVert \} \leq L_{f,grad} (\lVert \theta - \theta' \rVert + \lVert \phi - \phi' \rVert) \;\forall \theta,\theta',\phi,\phi'.
%%\end{equation}
%%\end{definition}

What \underline{solution concepts} are we looking at? Let's first define the notion of global optima for our min-max problem:
\begin{definition}[Global Optima]
\label{def:sol-concept}We define three equivalent notions of optimality:
\begin{enumerate}
    \item $(\theta^*, \phi^*)$ is a global min-max point, if for any $(\theta,\phi)$: $f(\theta^*, \phi) \leq f(\theta^*, \phi^*) \leq \max_{\phi'} f(\theta,\phi')$
    \item $(\theta^*, \phi^*)$ is a saddle point, if for any $(\theta,\phi)$: $f(\theta^*, y) \leq f(\theta^*, \phi^*) \leq f(x, \phi^*)$
    \item $(\theta^*, \phi^*)$ is a stationary point, if for any $(\theta,\phi)$: $\nabla_{\theta} f(\theta^*, \phi^*) = \nabla_{\phi} f(\theta^*, \phi^*) = 0 $.
\end{enumerate}
\end{definition}
It's well known that these three notions of optimality are not necessarily equivalent for an arbitrary nonconvex-nonconcave min-max problems. It's also true that a saddle point or global min-max point may not always exist for min-max problems. So, we assume that a saddle point always exists in our work.

\begin{assumption}[Existence of saddle points]
    \label{ass:saddle-exist}
    The objective function has at least one saddle point. Moreover, we also assume that for any fixed $\phi$, $\min_{\theta\in \mathbb{R}^{m}}f(\theta,\phi)$ has a non-empty solution set and a finite optimal value. Similarly, for any fixed $\theta$, $\max_{\phi\in \mathbb{R}^{n}}f(\theta, \phi)$ has a non-empty solution set and a finite optimal value.
\end{assumption}

\begin{lemma}[Lemma 2.1 in \cite{yang2020global}] If the objective function $f$ satisfies two-sided PŁ-condition, then all the three notions of global optimality are equivalent for our min-max problem:
    \[
    \text{(saddle point)} \iff \text{(global min-max)} \iff \text{(stationary point)}
    \]
\end{lemma}

\begin{assumption}
\label{ass:min-max-obj-assumptions}
The min-max objective function $f(\theta,\phi) $ is $(\mu_\theta, \mu_\phi)$-hidden-strongly-convex-hidden-strongly-concave, is $L_{f}$-Lipschitz and has $L_{f,grad}$-Lipschitz gradients.
\end{assumption}

\begin{lemma}[Proposition 4.1 in \cite{dorazio2025solving}]
    \label{lem:function-composition-pl-condition}
    Assume $f$ satisfies the $\mu$-PŁ condition, and let $\sigma_{\min}$ be a lower bound on the singular values of $J_{h(\theta)}=\frac{\partial h(\theta)}{\partial\theta}$. Then, we have $f\circ h$ satisfies $\mu\sigma_{\min}^{2}$-PŁ condition.
\end{lemma}

\begin{remark}(Why strong-convexity/strong-concavity?)
    We assume hidden-strongly-convex-hidden-strongly-concave for our min-max objective $f(\theta,\phi)$ so that, by Proposition 8 of \citeauthor{fatkhullin2023stochastic} \cite{fatkhullin2023stochastic}, we see that $f(\theta,\phi)$ satisfies PŁ-condition while keeping $\theta$ or $\phi$ fixed. That is, the min-max objective $f(\theta,\phi)$ satisfies 2-sided PŁ-condition \cite{yang2020global}. Another benefit is that we can use the convergence results of \citeauthor{yang2020global} \cite{yang2020global} for our min-max objective $f(\theta,\phi)$ in order to bound the path-length of the AltGDA iterates which will be crucial for analyzing degree of overparameterization needed for convergence.
\end{remark}



\begin{definition}[Two-layer Neural Network]
    \label{def:neural-net-def}
    We will be working with two-layer neural networks (commonly referred to as shallow neural networks). Specifically, such a network, $h$, can be specified as the following map:
    \begin{equation}
        x \mapsto W_2^{(h)} \psi(W_1^{(h)}x)
    \end{equation}
    where $x \in \mathbb{R}^{d_{0}^{(h)}}$, $W_1^{(h)} \in \mathbb{R}^{d_{1}^{(h)} \times d_{0}^{(h)}}$, and $W_2^{(h)}\in \mathbb{R}^{d_{2}^{(h)} \times d_{1}^{(h)}}$ and $\psi: \mathbb{R} \to \mathbb{R}$.
\end{definition}


\begin{definition}(Smoothness of neural network)
\label{def:smooth-neural-net}
 Let $\beta_h > 0$. A neural network $h: \mathbb{R}^{d_{0}^{(h)}} \to \mathbb{R}^{d_{2}^{(h)}}$ is $\beta_h$-smooth, if for all $u,v \in \mathbb{R}^{d_{0}^{(h)}}$, we have 
 \begin{equation}
     \label{eq:neural-net-smooth-def}
        \sigma_{\max}(\nabla h(u) - \nabla h(v)) \leq \beta_h \lVert u - v \rVert
 \end{equation}
\end{definition}

\begin{assumption}[Assumptions for the two-layer neural network]
    \label{ass:neural-net-act}
    We assume that the neural network function $h(\cdot)$ is twice-differentiable $\beta_h$-smooth. The activation function $\psi$ is twice-differentiable with $\psi(0) = 0, \sup_a \vert \dot\psi(a) \vert = \dot\psi_{\max} < \infty, \sup_a \vert \ddot \psi(a) \vert = \ddot \psi_{\max} < \infty$ and has a finite Hermite norm $\lVert \psi \rVert_{\mathcal{H}} < \infty$.

    We also assume that any data $(x, y)$ fed to the neural network satisfies $\lVert x \rVert = 1$ and $\lVert y\rVert \leq 1$.
\end{assumption}

\begin{remark}
    Although we assume the activation function $\psi$ to be twice-differentiable thereby excluding the commonly-used activation function ReLU, our results can still be applied to smooth approximations of ReLU such as Gaussian error Linear Units (GeLU) \cite{} or softplus \cite{} which have been empirically shown to exhibit comparable or better performance \cite{}.
\end{remark} 



==> related_work.tex <==
\subsection{Technical overview}

Several recent studies have explored this perspective.
In \cite{43}, the setting of hidden bilinear games was introduced, together with negative results showing that even when hidden bilinearity is present, gradient-descent-ascent can exhibit non-convergent behavior. 
Later, \cite{13} established an approximate minimax theorem for a class of two-player games where agents select neural networks as strategies, although no convergent training algorithm was provided.
The first positive convergence result appeared in \cite{44}, which established non-local convergence guarantees to the von Neumann solution under hidden strictly convex-concave structures, albeit only for continuous-time dynamics and under strong separability assumptions.

More recently, \cite{32} obtained the first global convergence guarantees in hidden games, again under continuous-time dynamics and for specific classes of convex-concave games (e.g., convex combinations of hidden one-dimensional latent games). 
This work introduced a dynamical system—Generalized Natural Gradient Flow—where the $\ell_2$ distance between the current and equilibrium latent profiles acts as a Lyapunov function. 
Building on this observation, \cite{?} proposed a flexible first-order method called \emph{preconditioned hidden gradient descent (PHGD)}, achieving convergence under minimal assumptions on the transformation between control and latent layers.
Subsequent extensions, such as \cite{?}, generalized PHGD ideas via surrogate losses, leveraging variants of Gauss-Newton (GN), Damped Gauss-Newton (DGN), and Levenberg-Marquardt (LM) methods; and further reductions were obtained in \cite{?} when the latent layer satisfies strong convexity via proximal Polyak–Łojasiewicz theory.

==> temp-input.tex <==
\clearpage
\section{Input-Optimization Min-Max Games}
\label{sec:input-games}
Here, we consider the input-optimization game between two neural networks $F_\theta$ and $G_\phi$ in hidden bilinear objective with $\ell_2$-regularization defined as follows for a given payoff matrix, $A$:
    \begin{equation}
    \label{eq:warmup-min-max-objective}
        \loss(\theta,\phi) = \opmin(\theta)^\top A \opmax(\phi) + \frac{\varepsilon}{2} \lVert \opmin(\theta) \rVert^2 - \frac{\varepsilon}{2} \lVert \opmax(\phi) \rVert^2
    \end{equation}
This game has been proposed by \cite{vlatakis2019poincare} and experimentally analyzed by \cite{sakos2023exploiting}.
Here, $\opmin_\theta$ and $\opmax_\phi$ are defined similar to Definition \ref{def:neural-net-def} as $\opmin(\theta) = W_2^{(\opmin)} \psi(W_1^{(\opmin)} \theta)$ and $\opmax(\phi) = W_{2}^{(\opmax)} \psi(W_1^{(\opmax)} \phi)$ but with parameters $\theta,\phi$ as inputs and randomly initalized $ W_k^{(\opmin)} \sim \mathcal{N}(0,\sigma_{k,\opmin}^2), W_k^{(\opmax)} \sim \mathcal{N}(0,(\sigma_{k,\opmax}^2)$, $k\in\{1,2\}$ along with differentiable activation function $\psi$ (e.g. GeLU). Therefore, the partial derivatives w.r.t. $\theta$ and $\phi$ will be as follows:
    \begin{align}
        \nabla_{\theta} f(\theta, \phi) & = (\nabla_\theta \opmin_\theta)^\top A \opmax(\phi) + \varepsilon (\nabla_\theta \opmin_\theta)^\top \opmin(\theta) \\
        \nabla_{\phi} f(\theta, \phi) & = J_{\opmax(\phi)}^\top A^\top \opmin(\theta) - \varepsilon J_{\opmax(\phi)}^\top \opmax(\phi)
    \end{align}
Using these and Lemma \ref{lem:potential-upper},  we can now bound $P_0$ as follows:
    \begin{align}
    \implies P_0 & \leq  \lVert \opmin(\theta_0) \rVert \cdot (\varepsilon L_{\loss} C_1 \sigma_{\max}(\nabla_\theta \opmin_{\theta_0}) + L_{\loss} C'_2 (1+\lambda)\sigma_{\max}(A) \sigma_{\max}(\nabla_\phi \opmax_{\phi_0})) \nonumber \\
        & + \lVert \opmax(\phi_0) \rVert \cdot (L_{\loss} C_1 \sigma_{\max}(A)\sigma_{\max}(\nabla_\theta \opmin_{\theta_0}) +\varepsilon C'_2(1+\lambda)\sigma_{\max}(\nabla_\phi \opmax_{\phi_0})) \label{eq:P_0-bound-1}
    \end{align}

Since we want to stay within the ball $\mathcal{B}((\theta_0,\phi_0), R)$, we can ensure $P_0 = \kappa R^2$ by controlling each term in Equation \eqref{eq:P_0-bound-1} accordingly that ultimately yields Theorem \ref{th:warmup-main-claim}. For this, we would additionally need to prove Lemma \ref{lem:warmup-jacobian-singular-smoothness-whp} as stated below. (Please see Appendix \ref{sec:appendix-input-games} for proof).

\begin{lemma}
    \label{lem:warmup-jacobian-singular-smoothness-whp}
    Consider a neural network $\opmin_\theta = \opmin(\theta) = W_{2}^{(\opmin)} \psi(W_{1}^{(\opmin)}\theta)$ as defined above. Say $\psi$ is the GeLU activation function, $d_{1}^{(\opmin)} \geq 256 \max\{ d_{0}^{(\opmin)}, d_{2}^{(\opmin)} \}$ and $\sigma_{1}^{(\opmin)} = \mathcal{O}\left((d_{1}^{(\opmin)} \lVert \theta \rVert^2)^{-0.5}\right)$. Then, w.p $\geq 1 - e^{-\Omega(d_{1}^{(\opmin)})}$, 
    \begin{enumerate}[label=(\roman*), nosep, leftmargin=*]
        \item the singular values of the Jacobian $\nabla_\theta \opmin_\theta$ are bounded as
            \begin{equation}
                \label{eq:warmup-jac-singular-bounds}
                \sigma_{\min}(\nabla_\theta \opmin_\theta) = \Omega\left(\sigma_{1,\opmin} \cdot \sigma_{2,\opmin} \cdot d_{1}^{(\opmin)}\right) \;\; \text{and} \;\; \sigma_{\max}(\nabla_\theta \opmin_\theta) = \mathcal{O}\left(\sigma_{1,\opmin} \cdot \sigma_{2,\opmin} \cdot d_{1}^{(\opmin)}\right)
            \end{equation}
        \item $\opmin(\theta)$ is $\beta_{\opmin}$-smooth where $\beta_{\opmin} = \Theta\left(\sigma_{1,\opmin}^2 \cdot \sigma_{2,\opmin} \cdot (d_{1}^{(\opmin)})^{3/2}\right)$.
    \end{enumerate}
\end{lemma}


\begin{theorem}
    \label{th:warmup-main-claim}
    Consider two neural networks $\opmin(\theta), \opmax(\phi)$ as defined in Lemma \ref{lem:warmup-jacobian-singular-whp} above. For the regularized hidden bilinear min-max objective $\loss(\theta,\phi)$ as defined in Equation \ref{eq:warmup-min-max-objective} above, AltGDA reaches  $\varepsilon$-saddle point w.p. $\geq 1 - e^{-\Omega(d_1^{(\opmin)})}$ if $(\theta_0,\phi_0)$ and standard deviations $\sigma_k^{(\opmin)}$ and $\sigma_k^{(\opmax)}$, $k\in\{1,2\}$ are chosen such that $\sigma_{k,F/G}=\Theta(\frac{\poly(1/d_1)}{\sigma_\max(A)})$:
    % \begin{align}
    %     \label{eq:warmup-main-claim}
    %     \sigma_{1}^{(\opmin)} = \mathcal{O}\left((d_{1}^{(\opmin)} \lVert \theta_0 \rVert^2)^{-0.5}\right) &, \quad \sigma_{1}^{(\opmax)} = \mathcal{O}\left((d_{1}^{(\opmax)} \lVert \phi_0 \rVert^2)^{-0.5}\right) \\
    %     (\sigma_{1}^{(\opmin)})^3 (\sigma_{2}^{(\opmin)})^2 = \mathcal{O}\left( (\varepsilon L_{\loss} (d_{1}^{(\opmin)})^{2.5})^{-1} \right) &, \quad (\sigma_{1}^{(\opmax)})^3 (\sigma_{2}^{(\opmax)})^2 = \mathcal{O}\left( (\varepsilon L_{\loss}d_{1}^{(\opmax)})^{2.5})^{-1}\right) \\
    %     (\sigma_1^{(\opmax)} \sigma_2^{(\opmax)}) ((\sigma_1^{(\opmin)})^2 \sigma_2^{(\opmin)}) & = \mathcal{O}\left((L_\loss (d_{1}^{(\opmin)})^{1.5}\sigma_{\max}(A))^{-1}\right) \\
    %     (\sigma_1^{(\opmin)} \sigma_2^{(\opmin)}) ((\sigma_1^{(\opmax)})^2 \sigma_2^{(\opmax)}) & = \mathcal{O}\left((L_\loss(d_{1}^{(\opmax)})^{1.5}\sigma_{\max}(A))^{-1}\right)
    % \end{align}
\end{theorem}
To our knowledge, this is the first fine-grained result that establishes an \( O(\epsilon) \)-approximate minimax solution for the hidden bilinear setting originally proposed by \textcite{vlatakis2019poincare}.


% \begin{theorem}
%     \label{th:warmup-main-claim}
%     Consider two neural networks $\opmin(\theta), \opmax(\phi)$ as defined in Lemma \ref{lem:warmup-jacobian-singular-whp} above. For the regularized hidden bilinear min-max objective $\loss(\theta,\phi)$ as defined in Equation \ref{eq:warmup-min-max-objective} above, AltGDA reaches  $\varepsilon$-saddle point w.p. $\geq 1 - e^{-\Omega(d_1^{(\opmin)})}$ if $(\theta_0,\phi_0)$ and standard deviations $\sigma_k^{(\opmin)}$ and $\sigma_k^{(\opmax)}$, $k\in\{1,2\}$ are chosen such that:
%     \begin{align}
%         \label{eq:warmup-main-claim}
%         \sigma_{1}^{(\opmin)} = \mathcal{O}\left((d_{1}^{(\opmin)} \lVert \theta_0 \rVert^2)^{-0.5}\right) &, \quad \sigma_{1}^{(\opmax)} = \mathcal{O}\left((d_{1}^{(\opmax)} \lVert \phi_0 \rVert^2)^{-0.5}\right) \\
%         (\sigma_{1}^{(\opmin)})^3 (\sigma_{2}^{(\opmin)})^2 = \mathcal{O}\left( (\varepsilon L_{\loss} (d_{1}^{(\opmin)})^{2.5})^{-1} \right) &, \quad (\sigma_{1}^{(\opmax)})^3 (\sigma_{2}^{(\opmax)})^2 = \mathcal{O}\left( (\varepsilon L_{\loss}d_{1}^{(\opmax)})^{2.5})^{-1}\right) \\
%         (\sigma_1^{(\opmax)} \sigma_2^{(\opmax)}) ((\sigma_1^{(\opmin)})^2 \sigma_2^{(\opmin)}) & = \mathcal{O}\left((L_\loss (d_{1}^{(\opmin)})^{1.5}\sigma_{\max}(A))^{-1}\right) \\
%         (\sigma_1^{(\opmin)} \sigma_2^{(\opmin)}) ((\sigma_1^{(\opmax)})^2 \sigma_2^{(\opmax)}) & = \mathcal{O}\left((L_\loss(d_{1}^{(\opmax)})^{1.5}\sigma_{\max}(A))^{-1}\right)
%     \end{align}
% \end{theorem}
